Stabilizing RNN Gradients through Pre-training

Numerous theories of learning propose to prevent the gradient from exponential growth with depth or time, to stabilize and improve training. Typically, these analyses are conducted on feed-forward fully-connected neural networks or simple single-layer recurrent neural networks, given their mathematical tractability. In contrast, this study demonstrates that pre-training the network to local stability can be effective whenever the architectures are too complex for an analytical initialization. Furthermore, we extend known stability theories to encompass a broader family of deep recurrent networks, requiring minimal assumptions on data and parameter distribution, a theory we call the Local Stability Condition (LSC). Our investigation reveals that the classical Glorot, He, and Orthogonal initialization schemes satisfy the LSC when applied to feed-forward fully-connected neural networks. However, analysing deep recurrent networks, we identify a new additive source of exponential explosion that emerges from counting gradient paths in a rectangular grid in depth and time. We propose a new approach to mitigate this issue, that consists on giving a weight of a half to the time and depth contributions to the gradient, instead of the classical weight of one. Our empirical results confirm that pre-training both feed-forward and recurrent networks, for differentiable, neuromorphic and state-space models to fulfill the LSC, often results in improved final performance. This study contributes to the field by providing a means to stabilize networks of any complexity. Our approach can be implemented as an additional step before pre-training on large augmented datasets, and as an alternative to finding stable initializations analytically.

==> sections/old_material.tex <==
\newpage

\section{\orange{Possibly to remove from the final paper}}



\begin{table*}
\centering
\begin{tabular}{lcccccc}
%  & \multicolumn{3}{l}{ALIF} \\
ALIF & \\
\hline
\rule{0pt}{1.3\normalbaselineskip} task & \multicolumn{2}{c}{sl-MNIST \uparrow} & \multicolumn{2}{c}{SHD \uparrow}  & \multicolumn{2}{c}{PTB \downarrow}  \\
 & val & test & val & test & val & test \\
\hline
\hline
no LSC            &  $92.77\pm0.48$ &  $92.69\pm0.54$ &  $\textbf{95.62}\pm1.8$ &  $\textbf{84.67}\pm\textbf{0.68}$ &  $132.23\pm0.69$ &  $120.3\pm0.84$ \\
LSC_1             &  $91.08\pm3.98$ &  $91.19\pm3.63$ &  $84.05\pm9.36$ &  $75.11\pm3.7$ &  $131.83\pm\textbf{0.05}$ &  $120.72\pm0.21$ \\
LSC_2             &  $63.72\pm16.43$ &  $63.65\pm16.79$ &  $88.78\pm3.13$ &  $81.48\pm2.7$ &  $134.28\pm0.26$ &  $122.67\pm\textbf{0.12}$ \\
LSC_\infty        &  $77.97\pm13.92$ &  $77.64\pm13.86$ &  $62.78\pm15.15$ &  $60.11\pm13.54$ &  $131.73\pm2.3$ &  $120.08\pm2.28$ \\
\hline
\hline
LSC_2 + g         &  $72.54\pm11.1$ &  $72.24\pm11.48$ &  $89.52\pm2.89$ &  $80.54\pm1.52$ &  - &  None \\
LSC_2 + b         &  $\textbf{92.86}\pm1.04$ &  $\textbf{92.81}\pm0.99$ &  $92.51\pm4.52$ &  $83.78\pm4.02$ &  - &  None \\
LSC_2 + s         &  $91.34\pm1.55$ &  $91.65\pm1.67$ &  $88.48\pm7.36$ &  $80.89\pm5.99$ &  $134.28\pm0.62$ &  $122.38\pm0.37$ \\
LSC_2 + c         &  - &  None &  - &  None &  $133.83\pm0.71$ &  $122.43\pm1.08$ \\
\hline
\hline
$\beta$ no LSC    &  $88.89\pm1.07$ &  $88.78\pm1.22$ &  $95.12\pm1.15$ &  $79.79\pm0.76$ &  $128.85\pm2.51$ &  $117.9\pm1.66$ \\
$\beta$ LSC_2     &  $89.29\pm\textbf{0.4}$ &  $89.45\pm\textbf{0.19}$ &  $94.1\pm0.86$ &  $78.84\pm1.3$ &  $128.68\pm3.13$ &  $117.03\pm2.55$ \\
$\beta$ LSC_2 + g &  $89.32\pm0.5$ &  $89.02\pm0.81$ &  $94.08\pm0.62$ &  $78.97\pm1.58$ &  $126.62\pm1.7$ &  $116.25\pm1.07$ \\
$\beta$ LSC_2 + b &  $89.28\pm0.58$ &  $89.14\pm0.96$ &  $94.81\pm\textbf{0.6}$ &  $79.99\pm1.12$ &  $\textbf{125.91}\pm1.22$ &  $\textbf{115.58}\pm0.55$ \\
$\beta$ LSC_2 + s &  $89.62\pm0.54$ &  $89.33\pm0.68$ &  $94.9\pm1.16$ &  $79.01\pm1.11$ &  $136.13\pm10.41$ &  $125.14\pm11.49$ \\
$\beta$ LSC_2 + c &  - &  None &  - &  None &  $131.03\pm7.01$ &  $120.62\pm8.51$ \\
\hline
\hline
LSC_2^{(d)}       &  $80.42\pm19.13$ &  $80.25\pm19.48$ &  $75.07\pm18.99$ &  $67.81\pm14.05$ &  - &  None \\
LSC_2^{(dr)}      &  $90.68\pm1.78$ &  $90.88\pm2.08$ &  $90.06\pm2.93$ &  $79.34\pm1.47$ &  - &  None \\
\bottomrule
\hline
\end{tabular}
\caption{\textbf{ALIF performance with and without LSC pre-training.} \red{I'm completing the tables with new experiments, so, there is a mismatch with the caption, old ones in the appendix.}
The metric reported for sl-MNIST and SHD is the accuracy, the higher the better, while for PTB is perplexity, the lower the better. On the left of the forward slash we have validation while on the right we have test mean and standard deviation. The ALIF can improve performance with the LSC pre-training, especially when the matrix norm induced by the $p=1$ norm is used ($LSC_1$). Using a 0.5 probability Bernouilli noise at the input during the LSC pre-training ($LSC_2+b$) seems especially beneficial for generalizing well on the test set, more than using standard Gaussian noise ($LSC_2+g$). Initializing the spike frequency adaptation $\beta$ with both positive and negative values, improves performance ($LSC_2\beta$). Further normalizing the depth transition derivative ($LSC_2^{(d)}$) and the readout ($LSC_2^{(dr)}$), improves training. \red{Explain beta reduction in std, and how beta helps only with language and not with classification. Write beta no LSC. } } \label{tab:alif}
\end{table*}




\subsection{LSC surpasses He on Efficientnet}

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{images/effnet_relu.pdf}
    \caption{\textbf{Stabilizing lower and upper bound in FFNs improves learning.} When the theoretically justified option of initialization is available, as it is the case for ReLU FFN networks with the He initialization, we can see that Glorot underperforms, but our stabilized bounds are competitive or outperform He. For an activation where a corresponding theoretically justified initialization is not available, like the sin, we see that Glorot experimentally outperforms He, but our bounds stabilized through pretraining, match or outperform He and Glorot. We see that stabilizing upper and lower bound (\textit{supsub}, in blue) results systematically in better learning, through activations and datasets. }
    \label{fig:effnplot}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{images/transfeff.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{images/rnns.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{images/rnns_layers.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{images/varag.png}
    \caption{\textbf{Gradient variance, and activity in a multi-layer ALIF at initialization.} Gradient variance and activity are computed in the first layer of a stack with 3 layers of 128 width. Input and outputs are two channels of samples from a standard normal distribution. Applying the LSC proves to result in more stable gradients, left panel, while different initializations can easily result in exponentially exploding gradients, right panel, even when the activity appears comparable.}
    \label{fig:varag}
\end{figure}



\subsection{LSC effect on LSTM and ALIF weight distributions}

Once the effect of the LSC on initialization and training is understood, we want to clarify what are the resulting weight distributions have become. Given that the transition derivatives have a complex dependence on the weights, the resulting distributions don't seem to have a simple intuitive explanation. We can see in Fig. \ref{fig:weightshist} the effect of pre-training the LSTM and ALIF to satisfy the LSC for $p=1, 2, \infty$, on the sl-MNIST task. The LSTM was closer to satisfy the LSC for $p=2$ with the default initialization, so there is only a minor change in the recurrent connections $U_j$, and in the input connections $W_{j,l}$ for that case, while there is a starker widening of the distributions for $p\neq2$. On the ALIF we can see a minor shift of the spike frequency adaptation $\beta_l$ values, and a starker shift and widening of the equilibrium threshold $b_l^\vartheta$. The remaining weight distributions can be seen in App.~\ref{app:weightdist}.

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{images/weights_aliflstm_sl-MNIST.pdf}
    \caption{\textbf{Effect of LSC pre-training on weight distribution.} LSTM and ALIF pre-trained to satisfy the LSC on the sl-MNIST task, for different $p$ matrix norms. The LSTM was already close to satisfy the LSC for $p=2$ with the default initialization, so we  only observe a subtle smoothing for $p=2$, but a starker difference is observed for $p=\infty$. The changes on ALIF distributions are more noticeable, especially we see a widening for the equilibrium threshold $b_l^\vartheta$ distribution, and an unclear reshuffling of the spike adaptation frequency $\beta_l^\vartheta$ distribution.}
    \label{fig:weightshist}
\end{figure}



\begin{table*}[]
\centering  
\begin{tabular}{lcccccc}
%  & \multicolumn{3}{l}{ALIF} \\
LSTM & \\
\hline
\rule{0pt}{1.3\normalbaselineskip} task & \multicolumn{2}{c}{sl-MNIST \uparrow} & \multicolumn{2}{c}{SHD \uparrow}  & \multicolumn{2}{c}{PTB \downarrow}  \\
 & val & test & val & test & val & test \\
\hline
\hline
no LSC            &  $95.57\pm0.43$ &  $95.43\pm0.44$ &  $97.98\pm0.44$ &  $86.68\pm1.0$ &  $118.35\pm0.56$ &  $107.18\pm0.57$ \\
LSC_1             &  $95.81\pm\textbf{0.12}$ &  $95.55\pm\textbf{0.09}$ &  $97.85\pm0.58$ &  $86.62\pm1.16$ &  $122.35\pm0.73$ &  $115.14\pm0.74$ \\
LSC_2             &  $95.84\pm0.32$ &  $95.6\pm0.31$ &  $97.92\pm0.74$ &  $84.9\pm2.03$ &  $123.76\pm1.46$ &  $115.74\pm2.11$ \\
LSC_\infty        &  $95.63\pm0.39$ &  $95.39\pm0.36$ &  $97.33\pm0.49$ &  $84.78\pm1.03$ &  $\textbf{114.55}\pm\textbf{0.37}$ &  $\textbf{105.27}\pm\textbf{0.39}$ \\
\hline
\hline
LSC_2 + g         &  $\textbf{95.97}\pm0.3$ &  $95.72\pm0.18$ &  $\textbf{98.37}\pm1.19$ &  $86.55\pm2.23$ &  $123.08\pm1.03$ &  $115.18\pm1.6$ \\
LSC_2 + b         &  $95.58\pm0.64$ &  $95.4\pm0.83$ &  $97.33\pm0.65$ &  $86.65\pm\textbf{0.36}$ &  $122.08\pm2.45$ &  $113.66\pm2.07$ \\
LSC_2 + s         &  $95.84\pm0.41$ &  $\textbf{95.8}\pm0.12$ &  $97.98\pm0.54$ &  $87.02\pm1.11$ &  $120.9\pm2.02$ &  $112.45\pm2.46$ \\
LSC_2 + c         &  - &  None &  - &  None &  $122.02\pm1.68$ &  $114.25\pm1.5$ \\
\hline
\hline
LSC_2^{(d)}       &  $95.6\pm0.36$ &  $95.57\pm0.33$ &  $97.92\pm\textbf{0.37}$ &  $\textbf{87.58}\pm1.39$ &  $121.11\pm2.31$ &  $113.09\pm2.99$ \\
LSC_2^{(dr)}      &  $95.89\pm0.15$ &  $95.71\pm0.12$ &  $97.79\pm0.75$ &  $85.96\pm0.56$ &  - &  None \\
\bottomrule
\hline
\end{tabular}
\caption{\textbf{LSTM performance with and without LSC pre-training.} The LSTM can improve performance with the LSC pre-training, especially when the matrix norm induced by the $p=1$ norm is used ($LSC_1$). Using Bernouilli noise at the input during the LSC pre-training ($LSC_2+b$) seems especially beneficial for generalizing well on the test set, more than using standard Gaussian noise ($LSC_2+g$). Further normalizing the depth transition derivative ($LSC_2^{(d)}$) and the readout ($LSC_2^{(dr)}$), has a positive effect on training.} \label{tab:lstm}
\end{table*}



\newpage
\clearpage
\section{Old tables}



\begin{table*}[h]
\centering  
\begin{tabular}{lccc}
LSTM & \\
\hline
 & sl-MNIST \uparrow & SHD \uparrow & PTB \downarrow  \\
\hline
\hline
no LSC                        &  94.82\pm0.23/94.74\pm0.24 &  94.08\pm6.6/81.38\pm6.19 &  \textbf{134.25}\pm0.74/\textbf{126.45}\pm0.66 \\
LSC_1          &  \textbf{95.59}\pm\textbf{0.14}/\textbf{95.52}\pm0.21 &  \textbf{98.68}\pm0.93/86.19\pm1.66 &  140.47\pm\textbf{0.41}/131.71\pm0.72 \\
LSC_2          &  94.89\pm0.16/94.78\pm0.25 &  97.53\pm1.73/\textbf{86.61}\pm1.52 &  143.99\pm1.67/134.98\pm1.07 \\
LSC_\infty     &  95.23\pm0.32/95.08\pm0.28 &  98.52\pm0.83/86.12\pm1.38 &  134.47\pm1.44/127.15\pm1.51 \\
\hline
\hline
LSC_2 + g      &  94.85\pm0.15/94.74\pm0.18 &  97.53\pm1.12/86.56\pm2.06 &  - \\
LSC_2 + b      &  94.93\pm0.16/94.86\pm0.12 &  97.86\pm\textbf{0.63}/85.45\pm\textbf{0.63} &  - \\
LSC_2 + s      &  95.05\pm0.2/94.85\pm\textbf{0.07} &  - &  144.16\pm1.14/135.12\pm1.26 \\
\hline
\hline
LSC_2^{(d)}    &  94.94\pm0.27/94.8\pm0.42 &  95.72\pm6.41/83.82\pm6.71 &  140.65\pm1.37/131.53\pm0.75 \\
LSC_2^{(dr)}   &  94.9\pm0.18/94.97\pm0.23 &  98.52\pm1.73/86.06\pm1.52 &  - \\
\bottomrule
\hline
\end{tabular}
\caption{\textbf{LSTM performance with and without LSC pre-training.} The LSTM can improve performance with the LSC pre-training, especially when the matrix norm induced by the $p=1$ norm is used ($LSC_1$). Using Bernouilli noise at the input during the LSC pre-training ($LSC_2+b$) seems especially beneficial for generalizing well on the test set, more than using standard Gaussian noise ($LSC_2+g$). Further normalizing the depth transition derivative ($LSC_2^{(d)}$) and the readout ($LSC_2^{(dr)}$), has a positive effect on training.} \label{tab:lstm}
\end{table*}



\begin{table*}
\centering
% \tiny
\begin{tabular}{lcccccc}
%  & \multicolumn{3}{l}{ALIF} \\
% ALIF & \\
\hline
 & & sl-MNIST & & SHD & & PTB \\
 & val & test & val & test & val & test \\
% comments & & & & & & \\
\midrule
no LSC            &  87.93\pm10.05 &  87.94\pm10.12 &  \textbf{98.19}\pm0.63 &  85.73\pm1.52 &  157.1\pm0.52 &  146.37\pm0.63 \\
LSC_1             &  93.02\pm2.3 &  93.13\pm2.28 &  - &  None &  154.72\pmnan &  143.78\pmnan \\
LSC_2             &  80.5\pm14.92 &  80.55\pm15.26 &  77.47\pm28.16 &  71.01\pm20.6 &  - &  None \\
LSC_\infty        &  84.33\pm14.71 &  84.27\pm15.06 &  79.77\pm11.49 &  74.88\pm8.68 &  - &  None \\
LSC_2 + g         &  86.46\pm5.31 &  86.39\pm5.19 &  82.07\pm24.0 &  74.32\pm12.85 &  - &  None \\
LSC_2 + b         &  94.62\pm0.14 &  94.63\pm0.3 &  95.56\pm2.17 &  \textbf{86.1}\pm1.52 &  - &  None \\
LSC_2 + s         &  87.19\pm15.0 &  87.06\pm15.04 &  - &  None &  - &  None \\
LSC_2 + c         &  - &  None &  - &  None &  - &  None \\
$\beta$ no LSC    &  92.29\pm0.45 &  92.02\pm0.29 &  97.7\pm1.57 &  80.16\pm\textbf{0.71} &  135.97\pm0.36 &  127.29\pm0.43 \\
% $\beta$ no LSC    &  92.29\pm0.45 &  92.02\pm0.29 &  97.7\pm1.57 &  80.16\pm\textbf{0.71} &  135.97\pm0.36 &  127.29\pm0.43 \\
% $\beta$ LSC_2     &  91.97\pm \textbf{0.13} &  91.98\pm \textbf{0.13} &  96.38 \pm 0.66 &  80.86 \pm 1.5 &  \textbf{134.51} \pm 0.67 &  125.79 \pm 0.75 \\
% $\beta$ LSC_2 + g &  92.24\pm0.27 &  92.14\pm0.2 &  96.55\pm0.83 &  80.53\pm0.97 &  134.61\pm\textbf{0.23} &  125.88\pm\textbf{0.17} \\
% $\beta$ LSC_2 + b &  92.02\pm0.24 &  91.89\pm0.2 &  96.71\pm\textbf{0.54} &  79.37\pm1.31 &  134.53\pm0.7 &  \textbf{125.76}\pm0.54 \\
% $\beta$ LSC_2 + s &  91.89\pm0.38 &  91.9\pm0.29 &  - &  None &  135.25\pm0.57 &  126.48\pm0.62 \\
$\beta$ LSC_2 + c &  - &  None &  - &  None &  - &  None \\
LSC_2^{(d)}       &  94.33\pm0.92 &  94.32\pm0.94 &  91.78\pm3.26 &  80.75\pm1.37 &  - &  None \\
LSC_2^{(dr)}      &  \textbf{94.66}\pm0.37 &  \textbf{94.87}\pm0.25 &  - &  None &  - &  None \\
\bottomrule
\hline
\end{tabular}
\caption{\textbf{ALIF performance with and without LSC pre-training.}
The metric reported for sl-MNIST and SHD is the accuracy, the higher the better, while for PTB is perplexity, the lower the better. On the left of the forward slash we have validation while on the right we have test mean and standard deviation. The ALIF can improve performance with the LSC pre-training, especially when the matrix norm induced by the $p=1$ norm is used ($LSC_1$). Using a 0.5 probability Bernouilli noise at the input during the LSC pre-training ($LSC_2+b$) seems especially beneficial for generalizing well on the test set, more than using standard Gaussian noise ($LSC_2+g$). Initializing the spike frequency adaptation $\beta$ with both positive and negative values, improves performance ($LSC_2\beta$). Further normalizing the depth transition derivative ($LSC_2^{(d)}$) and the readout ($LSC_2^{(dr)}$), improves training. \red{Explain beta reduction in std, and how beta helps only with language and not with classification. Write beta no LSC.}} \label{tab:alif}
\end{table*}


\newpage
\clearpage
\section{Weight distributions after LSC pretraining}
\label{app:weightdist}

Here we report how the weights distributions where changed after pre-training LSTM and ALIF to satisfy the LSC, on the sl-MNIST task.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/weights_LSTM_sl-MNIST_gbFalse.pdf}
    \includegraphics[width=\textwidth]{images/weights_ALIF_sl-MNIST_gbFalse.pdf}
\caption{\textbf{LSTM and ALIF weight distributions before and after applying the LSC.} The LSC pre-training is done on the sl-MNIST dataset. Upper block of panels show LSTM weights distributions. We see that $p=2$ leaves the weights distributions closer to the default initialization, given that the latter is a variance based FFN initialization, therefore, essentially $p=2$ in nature. The LSC that departs the most from the default is $p=\infty$. The effect on ALIF is starker, since the default initialization was further away from stability. Essentially we see a sharpening of the recurrent and input weights distributions, and a widening of the equilibrium threshold distribution, for all $p$.}
    \label{fig:my_label}
\end{figure}

% \begin{figure}
%     \centering
% \caption{Caption}
%     \label{fig:my_label}
% \end{figure}



\subsection{Experimentally LSC stabilizes gradients at initialization}

First of all, we need to confirm that the LSC provides the desired stabilization effect on the gradients at initialization, before assessing the effect on training. We can observe in Fig. \ref{fig:varag}, how a bad initialization can easily result in a variance of the update that grows exponentially in time, even for a neuron activity that seems comparable, in contrast with the gradients variance after applying the LSC. Since the gradient accumulates from the last time step backwards, the explosion is backwards in data time $t$. We conclude that the LSC is sufficient to prevent such an explosion experimentally at initialization.





\begin{table}[h]
\centering
\resizebox{.5\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
 \textbf{Depth 3 LRU} & \textbf{\shortstack{validation \\ perplexity} } & \textbf{\shortstack{test \\ perplexity} } \\
\midrule
default & $\textbf{136.10}~\pm~\textbf{0.61}$ & $126.61~\pm~0.82$ \\
$\rho_t=1$ & $156.25~\pm~1.01$ & $143.35~\pm~1.30$ \\
$\rho_t=0.5$ & $145.94~\pm~0.79$ & $132.86~\pm~\textbf{0.43}$ \\
$\overline{\rho}_t=0.5$ & $136.86~\pm~0.83$ & $\textbf{126.29}~\pm~0.69$ \\
default + clip & $\textbf{136.10}~\pm~0.61$ & $126.61~\pm~0.82$ \\
$\rho_t=1$ + clip & $158.28~\pm~0.56$ & $144.89~\pm~\textbf{0.44}$ \\
$\rho_t=0.5$ + clip & $145.67~\pm~\textbf{0.05}$ & $132.66~\pm~0.63$ \\
$\overline{\rho}_t=0.5$ + clip & $136.86~\pm~0.83$ & $\textbf{126.29}~\pm~0.69$ \\
\bottomrule
\toprule
 \textbf{Depth 6 LRU} & \textbf{\shortstack{validation \\ perplexity} } & \textbf{\shortstack{test \\ perplexity} } \\
\midrule
default & $133.67~\pm~0.86$ & $123.54~\pm~0.88$ \\
$\rho_t=1$ & $157.34~\pm~1.00$ & $144.83~\pm~0.87$ \\
$\rho_t=0.5$ & $140.93~\pm~1.03$ & $129.28~\pm~\textbf{0.31}$ \\
$\overline{\rho}_t=0.5$ & $\textbf{132.99}~\pm~\textbf{0.50}$ & $\textbf{122.46}~\pm~1.26$ \\
default + clip & $133.67~\pm~0.86$ & $123.54~\pm~0.88$ \\
$\rho_t=1$ + clip & $159.72~\pm~1.18$ & $146.61~\pm~1.88$ \\
$\rho_t=0.5$ + clip & $141.71~\pm~0.74$ & $129.29~\pm~\textbf{0.55}$ \\
$\overline{\rho}_t=0.5$ + clip & $\textbf{132.84}~\pm~\textbf{0.72}$ & $\textbf{121.95}~\pm~0.62$ \\
\bottomrule
\end{tabular}



}
\caption{\orange{\textbf{Pre-training has a stronger effect than gradient clipping.} Validation and test results from the experiments in Fig.~\ref{fig:lru}, for the LRU state-space model trained on the PTB language modeling task. }}
\label{tab:lru}
\end{table}

==> sections/old_tables.tex <==

\newpage
\clearpage
\section*{Old tables}

\red{This section will be removed in the submitted article.}

\section{06 May 2023}

% 10 -> 
\begin{table*}[h]
\centering

\begin{tabular}{llrccc}
\toprule
 & & \textbf{task} & \textbf{sl-MNIST} $\uparrow$ & \textbf{SHD} $\uparrow$ & \textbf{PTB} $\downarrow$ \\
\textbf{net} & \textbf{LSC} & & & & \\
\\ \toprule\midrule 
 RNN $\sigma$ & $\rho_t=0.5$ & metric & $\textbf{29.38}\pm 6.65$ & $34.66\pm 8.30$ & $121.16\pm 3.85$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.492\pm 0.008$ & \scriptsize $0.496\pm 0.007$ & \scriptsize $0.492\pm 0.011$ \\
 & $\rho_t=1$ & metric & \sout{$24.18\pm 6.86$} & $38.16\pm \textbf{2.71}$ & \sout{$\textbf{113.31}\pm \textbf{1.71}$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize \sout{$0.971\pm 0.024$} & \scriptsize $1.019\pm 0.019$ & \scriptsize \sout{$0.889\pm 0.070$} \\
 & none & metric & $29.02\pm \textbf{2.00}$ & $\textbf{46.40}\pm 12.12$ & $120.77\pm 2.67$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.354\pm 0.002$ & \scriptsize $0.363\pm 0.001$ & \scriptsize $0.353\pm 0.000$ \\
\midrule
 RNN $ReLU$ & $\rho_t=0.5$ & metric & $\textbf{28.12}\pm 3.41$ & $35.46\pm 10.64$ & \sout{$237.47\pm 97.22$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.500\pm 0.003$ & \scriptsize $0.508\pm 0.003$ & \scriptsize \sout{$0.414\pm 0.001$} \\
 & $\rho_t=1$ & metric & $24.80\pm 5.44$ & \sout{$33.40\pm \textbf{5.63}$} & \sout{$238.82\pm 96.21$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.997\pm 0.009$ & \scriptsize \sout{$0.845\pm 0.177$} & \scriptsize \sout{$0.414\pm 0.001$} \\
 & none & metric & $23.51\pm \textbf{2.50}$ & $\textbf{39.84}\pm 5.91$ & $\textbf{173.67}\pm \textbf{3.21}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.317\pm 0.011$ & \scriptsize $1.349\pm 0.007$ & \scriptsize $0.760\pm 0.004$ \\
\midrule
 GRU & $\rho_t=0.5$ & metric & $\textbf{95.14}\pm 0.48$ & $\textbf{85.58}\pm \textbf{1.35}$ & $\textbf{103.12}\pm \textbf{0.25}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.488\pm 0.016$ & \scriptsize $0.491\pm 0.006$ & \scriptsize $0.499\pm 0.001$ \\
 & $\rho_t=1$ & metric & $95.04\pm 0.75$ & $84.10\pm 2.27$ & $103.41\pm 0.78$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.999\pm 0.004$ & \scriptsize $1.003\pm 0.005$ & \scriptsize $1.002\pm 0.004$ \\
 & none & metric & $94.79\pm \textbf{0.38}$ & $84.92\pm 2.05$ & $104.05\pm 0.53$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.710\pm 0.004$ & \scriptsize $0.719\pm 0.002$ & \scriptsize $0.694\pm 0.002$ \\
\midrule
 LSTM & $\rho_t=0.5$ & metric & $95.21\pm \textbf{0.24}$ & \sout{$\textbf{84.48}\pm \textbf{0.97}$} & $\textbf{108.83}\pm 1.65$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.503\pm 0.006$ & \scriptsize \sout{$0.536\pm 0.026$} & \scriptsize $0.511\pm 0.016$ \\
 & $\rho_t=1$ & metric & \sout{$\textbf{95.53}\pm 0.42$} & $83.95\pm 2.44$ & $109.33\pm \textbf{0.71}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize \sout{$0.955\pm 0.038$} & \scriptsize $0.997\pm 0.014$ & \scriptsize $1.000\pm 0.018$ \\
 & none & metric & $95.20\pm 0.95$ & $84.17\pm 2.19$ & $109.03\pm 3.03$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.876\pm 0.005$ & \scriptsize $0.887\pm 0.002$ & \scriptsize $0.847\pm 0.003$ \\
\midrule\midrule
ALIF$_{+}$ & $\rho_t=1$ & metric & \sout{$90.31\pm 1.22$} & \sout{$\textbf{82.11}\pm 3.01$} & \sout{$131.78\pm 1.68$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize \sout{$0.966\pm 0.009$} & \scriptsize \sout{$0.950\pm 0.102$} & \scriptsize \sout{$0.978\pm 0.208$} \\
 & none & metric & $\textbf{91.68}\pm \textbf{1.01}$ & $77.99\pm \textbf{2.68}$ & $\textbf{130.18}\pm \textbf{1.06}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $2.225\pm 0.033$ & \scriptsize $1.748\pm 0.016$ & \scriptsize $1.690\pm 0.022$ \\
\midrule
ALIF$_{\pm}$ & $\rho_t=1$ & metric & $\textbf{87.17}\pm 2.25$ & $74.19\pm 3.71$ & \sout{$\textbf{127.94}\pm \textbf{0.97}$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.999\pm 0.001$ & \scriptsize $1.000\pm 0.000$ & \scriptsize \sout{$0.876\pm 0.176$} \\
 & none & metric & $82.07\pm \textbf{1.12}$ & $\textbf{74.76}\pm \textbf{1.34}$ & $130.31\pm 3.05$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.212\pm 0.007$ & \scriptsize $1.130\pm 0.003$ & \scriptsize $1.094\pm 0.002$ \\
\midrule\bottomrule
\end{tabular}
\caption{\textbf{Effect of stabilization across tasks and networks.} The network preparation by pre-training to stability, generally helps performance, with $\rho_t=0.5$ generally being preferable over $\rho_t=1$ across tasks and networks, with networks of depth $d=2$. Here we report the test set results across three different tasks. Metrics are accuracy for sl-MNIST and SHD, the higher the better, and perplexity for PTB, the lower the better. The non-differentiable networks, were often unable to reach a target norm of $\rho_t=0.5$, but the preparation to $\rho_t=1$ was still often beneficial. \red{ The strike through the number means that it wasn't close enough to the target radius, where close enough means at a distance of $0.02$, and those experiments are currently running again.}}
\label{tab:lsctask}
\end{table*}




% 10 -> 10
\begin{table}[]
\centering

\begin{tabular}{llrccc}
\toprule
 & & \textbf{task} & \textbf{sl-MNIST} $\uparrow$ & \textbf{SHD} $\uparrow$ & \textbf{PTB} $\downarrow$ \\
\textbf{net} & \textbf{LSC} & & & & \\
\\ \toprule\midrule 
 RNN $\sigma$ & $\rho_t=0.5$ & metric & $11.19\pm 0.30$ & $\textbf{14.71}\pm \textbf{3.50}$ & \sout{$643.36\pm \textbf{0.63}$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.498\pm 0.003$ & \scriptsize $0.498\pm 0.002$ & \scriptsize \sout{$0.202\pm 0.001$} \\
 & $\rho_t=1$ & metric & $\textbf{11.45}\pm \textbf{0.16}$ & $9.45\pm 4.17$ & \sout{$\textbf{403.84}\pm 276.62$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.999\pm 0.019$ & \scriptsize $1.016\pm 0.019$ & \scriptsize \sout{$1.053\pm 0.064$} \\
 & none & metric & $11.30\pm 0.40$ & $12.90\pm 3.82$ & $643.23\pm 0.94$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.357\pm 0.002$ & \scriptsize $0.361\pm 0.001$ & \scriptsize $0.351\pm 0.001$ \\
\midrule
 RNN $ReLU$ & $\rho_t=0.5$ & metric & $17.15\pm 4.90$ & $\textbf{24.90}\pm 3.62$ & \sout{$585.56\pm 99.79$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.505\pm 0.008$ & \scriptsize $0.511\pm 0.003$ & \scriptsize \sout{$0.426\pm 0.002$} \\
 & $\rho_t=1$ & metric & $17.90\pm \textbf{2.04}$ & \sout{$18.77\pm \textbf{1.69}$} & 0 \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.002\pm 0.006$ & \scriptsize \sout{$0.859\pm 0.163$} & \scriptsize 0 \\
 & none & metric & $\textbf{19.63}\pm 6.60$ & $16.43\pm 3.51$ & $\textbf{500.04}\pm \textbf{94.49}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.323\pm 0.009$ & \scriptsize $1.341\pm 0.006$ & \scriptsize $0.769\pm 0.001$ \\
\midrule
 GRU & $\rho_t=0.5$ & metric & $\textbf{95.61}\pm \textbf{0.28}$ & $86.47\pm \textbf{0.60}$ & \sout{$651.71\pm 8.00$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.502\pm 0.002$ & \scriptsize $0.500\pm 0.002$ & \scriptsize \sout{$0.448\pm 0.002$} \\
 & $\rho_t=1$ & metric & $94.33\pm 1.31$ & $86.24\pm 2.38$ & \sout{$\textbf{249.92}\pm 268.44$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.999\pm 0.008$ & \scriptsize $1.016\pm 0.017$ & \scriptsize \sout{$0.822\pm 0.020$} \\
 & none & metric & $\textbf{95.61}\pm 0.38$ & $\textbf{87.81}\pm 1.56$ & $650.33\pm \textbf{1.17}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.695\pm 0.003$ & \scriptsize $0.702\pm 0.002$ & \scriptsize $0.687\pm 0.002$ \\
\midrule
 LSTM & $\rho_t=0.5$ & metric & $\textbf{95.65}\pm \textbf{0.35}$ & $82.04\pm \textbf{1.15}$ & $642.86\pm 1.05$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.501\pm 0.001$ & \scriptsize $0.506\pm 0.008$ & \scriptsize $0.509\pm 0.002$ \\
 & $\rho_t=1$ & metric & $53.70\pm 48.80$ & $\textbf{82.59}\pm 2.73$ & \sout{$\textbf{141.58}\pm 4.04$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.996\pm 0.006$ & \scriptsize $1.010\pm 0.007$ & \scriptsize \sout{$0.933\pm 0.035$} \\
 & none & metric & $74.92\pm 42.28$ & $67.71\pm 23.73$ & $644.18\pm \textbf{0.59}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.858\pm 0.002$ & \scriptsize $0.871\pm 0.001$ & \scriptsize $0.854\pm 0.001$ \\
\midrule\midrule
ALIF$_{+}$ & $\rho_t=1$ & metric & \sout{$\textbf{29.14}\pm 29.95$} & $\textbf{18.93}\pm 12.85$ & \sout{$\textbf{661.67}\pm 6.22$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize \sout{$0.799\pm 0.005$} & \scriptsize $0.995\pm 0.012$ & \scriptsize \sout{$0.620\pm 0.003$} \\
 & none & metric & $11.05\pm \textbf{0.28}$ & $18.85\pm \textbf{10.20}$ & $665.07\pm \textbf{1.72}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $2.281\pm 0.014$ & \scriptsize $1.663\pm 0.007$ & \scriptsize $1.650\pm 0.023$ \\
\midrule
ALIF$_{\pm}$ & $\rho_t=1$ & metric & $10.76\pm \textbf{0.80}$ & $14.23\pm 5.72$ & \sout{$662.17\pm 6.09$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.980\pm 0.014$ & \scriptsize $1.000\pm 0.001$ & \scriptsize \sout{$0.619\pm 0.002$} \\
 & none & metric & $\textbf{18.90}\pm 15.85$ & $\textbf{15.26}\pm \textbf{5.53}$ & $\textbf{661.85}\pm \textbf{0.89}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.090\pm 0.005$ & \scriptsize $0.979\pm 0.002$ & \scriptsize $0.973\pm 0.001$ \\
\midrule\bottomrule
\end{tabular}

\caption{Depth 5}
\label{tab:depth5}
\end{table}



\begin{table*}[h]
\centering
\addtolength{\leftskip} {-1cm}
\addtolength{\rightskip}{-1cm}
\resizebox{1.1\textwidth}{!}{%

% 9 -> 9

\begin{tabular}{llrcccc}
\toprule
 & & \textbf{depth} & 1 & 3 & 5 & 7 \\
\textbf{net} & \textbf{LSC} & & & & & \\
\\ \toprule\midrule 
 RNN $\sigma$ & $\rho_t=0.5$ & metric & $\textbf{41.29}\pm 3.82$ & $30.38\pm \textbf{6.97}$ & $\textbf{14.71}\pm \textbf{3.50}$ & $\textbf{7.99}\pm 3.43$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.504\pm 0.005$ & \scriptsize $0.500\pm 0.003$ & \scriptsize $0.498\pm 0.002$ & \scriptsize $0.500\pm 0.002$ \\
 & $\rho_t=1$ & metric & $37.64\pm \textbf{3.55}$ & $24.52\pm 8.06$ & $9.45\pm 4.17$ & $4.94\pm 0.16$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.992\pm 0.016$ & \scriptsize $1.019\pm 0.077$ & \scriptsize $1.016\pm 0.019$ & \scriptsize $1.003\pm 0.004$ \\
 & none & metric & $38.20\pm 6.84$ & $\textbf{30.47}\pm 13.34$ & $12.90\pm 3.82$ & $5.06\pm \textbf{0.16}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.366\pm 0.001$ & \scriptsize $0.362\pm 0.001$ & \scriptsize $0.361\pm 0.001$ & \scriptsize $0.361\pm 0.000$ \\
\midrule
 RNN $ReLU$ & $\rho_t=0.5$ & metric & $37.48\pm 9.97$ & $26.52\pm 6.23$ & $\textbf{24.90}\pm 3.62$ & $18.27\pm 2.88$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.512\pm 0.003$ & \scriptsize $0.511\pm 0.003$ & \scriptsize $0.511\pm 0.003$ & \scriptsize $0.512\pm 0.001$ \\
 & $\rho_t=1$ & metric & \sout{$37.92\pm \textbf{4.14}$} & $28.24\pm \textbf{5.18}$ & \sout{$18.77\pm \textbf{1.69}$} & \sout{$\textbf{18.32}\pm 5.13$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize \sout{$0.821\pm 0.199$} & \scriptsize $1.004\pm 0.010$ & \scriptsize \sout{$0.859\pm 0.163$} & \scriptsize \sout{$0.731\pm 0.007$} \\
 & none & metric & $\textbf{39.06}\pm 10.85$ & $\textbf{34.19}\pm 5.98$ & $16.43\pm 3.51$ & $15.59\pm \textbf{2.31}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.355\pm 0.004$ & \scriptsize $1.346\pm 0.003$ & \scriptsize $1.341\pm 0.006$ & \scriptsize $1.339\pm 0.005$ \\
\midrule
 GRU & $\rho_t=0.5$ & metric & \sout{$\textbf{84.53}\pm 2.13$} & $\textbf{86.05}\pm 2.98$ & $86.47\pm \textbf{0.60}$ & $\textbf{86.12}\pm 2.35$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize \sout{$0.461\pm 0.006$} & \scriptsize $0.495\pm 0.009$ & \scriptsize $0.500\pm 0.002$ & \scriptsize $0.500\pm 0.002$ \\
 & $\rho_t=1$ & metric & $76.01\pm 3.56$ & $84.29\pm \textbf{1.79}$ & $86.24\pm 2.38$ & \sout{$85.87\pm \textbf{1.52}$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.993\pm 0.006$ & \scriptsize $1.006\pm 0.005$ & \scriptsize $1.016\pm 0.017$ & \scriptsize \sout{$1.031\pm 0.021$} \\
 & none & metric & $84.01\pm \textbf{0.91}$ & $86.01\pm 2.48$ & $\textbf{87.81}\pm 1.56$ & $84.72\pm 3.89$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.751\pm 0.002$ & \scriptsize $0.710\pm 0.002$ & \scriptsize $0.702\pm 0.002$ & \scriptsize $0.699\pm 0.002$ \\
\midrule
 LSTM & $\rho_t=0.5$ & metric & \sout{$\textbf{83.67}\pm \textbf{1.24}$} & $\textbf{86.75}\pm \textbf{0.44}$ & $82.04\pm \textbf{1.15}$ & $57.13\pm 35.78$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize \sout{$0.528\pm 0.006$} & \scriptsize $0.514\pm 0.014$ & \scriptsize $0.506\pm 0.008$ & \scriptsize $0.504\pm 0.003$ \\
 & $\rho_t=1$ & metric & \sout{$67.26\pm 25.88$} & $84.15\pm 1.81$ & $\textbf{82.59}\pm 2.73$ & \sout{$\textbf{70.54}\pm 25.93$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize \sout{$0.978\pm 0.032$} & \scriptsize $1.005\pm 0.007$ & \scriptsize $1.010\pm 0.007$ & \scriptsize \sout{$1.030\pm 0.028$} \\
 & none & metric & $76.69\pm 9.27$ & $83.98\pm 2.20$ & $67.71\pm 23.73$ & $40.56\pm \textbf{19.39}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $0.914\pm 0.003$ & \scriptsize $0.879\pm 0.002$ & \scriptsize $0.871\pm 0.001$ & \scriptsize $0.869\pm 0.002$ \\
\midrule\midrule
ALIF$_{+}$ & $\rho_t=1$ & metric & $\textbf{77.98}\pm \textbf{1.02}$ & $53.58\pm 32.72$ & $\textbf{18.93}\pm 12.85$ & \sout{$\textbf{5.93}\pm 1.24$} \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.003\pm 0.005$ & \scriptsize $1.012\pm 0.032$ & \scriptsize $0.995\pm 0.012$ & \scriptsize \sout{$0.913\pm 0.128$} \\
 & none & metric & $76.94\pm 2.06$ & $\textbf{62.43}\pm \textbf{4.44}$ & $18.85\pm \textbf{10.20}$ & $4.69\pm \textbf{0.58}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.853\pm 0.023$ & \scriptsize $1.701\pm 0.011$ & \scriptsize $1.663\pm 0.007$ & \scriptsize $1.656\pm 0.007$ \\
\midrule
ALIF$_{\pm}$ & $\rho_t=1$ & metric & $\textbf{67.74}\pm \textbf{1.52}$ & $\textbf{66.96}\pm 9.64$ & $14.23\pm 5.72$ & $\textbf{7.88}\pm 3.94$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.000\pm 0.003$ & \scriptsize $1.001\pm 0.002$ & \scriptsize $1.000\pm 0.001$ & \scriptsize $1.000\pm 0.001$ \\
 & none & metric & $66.83\pm 4.23$ & $64.05\pm \textbf{5.50}$ & $\textbf{15.26}\pm \textbf{5.53}$ & $4.90\pm \textbf{0.17}$ \\
 & \scriptsize & \scriptsize $\rho$ & \scriptsize $1.460\pm 0.007$ & \scriptsize $1.016\pm 0.001$ & \scriptsize $0.979\pm 0.002$ & \scriptsize $0.933\pm 0.001$ \\
\midrule\bottomrule
\end{tabular}

}
\caption{\textbf{Effect of stabilization across depths and networks.} Networks of different depths are trained on the SHD task. All seem to benefit of the stabilization technique used before training, and  especially when the networks are prepared to have a $\rho_t=0.5$ as the networks become deeper. }
\label{tab:lscdepth}
\end{table*}


\newpage
\clearpage
\section{09 May 2023}



% 11 -> 8
\begin{table*}[h]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN$\sigma$&$\rho_t=0.5$&metric&$\textbf{29.38}\pm6.65$&$34.66\pm8.30$&$117.33\pm6.06$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.492\pm0.008$&\scriptsize$0.496\pm0.007$&\scriptsize$0.492\pm0.011$\\
&$\rho_t=1$&metric&$23.94\pm3.82$&$38.31\pm\textbf{2.73}$&\sout{$\textbf{112.51}\pm\textbf{1.66}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.970\pm0.029$&\scriptsize$1.019\pm0.019$&\scriptsize\sout{$0.889\pm0.070$}\\
&none&metric&$29.02\pm\textbf{2.00}$&$\textbf{46.40}\pm12.12$&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354\pm0.002$&\scriptsize$0.363\pm0.001$&\scriptsize0\\
\midrule
RNN$ReLU$&$\rho_t=0.5$&metric&$\textbf{28.12}\pm3.41$&$35.46\pm10.64$&\sout{$247.21\pm97.18$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500\pm0.003$&\scriptsize$0.508\pm0.003$&\scriptsize\sout{$0.414\pm0.001$}\\
&$\rho_t=1$&metric&$24.80\pm5.44$&\sout{$33.50\pm\textbf{5.65}$}&\sout{$237.47\pm97.22$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.997\pm0.009$&\scriptsize\sout{$0.845\pm0.177$}&\scriptsize\sout{$0.414\pm0.001$}\\
&none&metric&$23.51\pm\textbf{2.50}$&$\textbf{39.84}\pm5.91$&$\textbf{173.67}\pm\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317\pm0.011$&\scriptsize$1.349\pm0.007$&\scriptsize$0.760\pm0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\textbf{95.10}\pm0.55$&$\textbf{85.58}\pm\textbf{1.35}$&$\textbf{103.12}\pm0.25$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.488\pm0.016$&\scriptsize$0.491\pm0.006$&\scriptsize$0.499\pm0.001$\\
&$\rho_t=1$&metric&$95.04\pm0.75$&$83.59\pm2.70$&$103.41\pm0.78$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999\pm0.004$&\scriptsize$1.003\pm0.005$&\scriptsize$1.002\pm0.004$\\
&none&metric&$94.78\pm\textbf{0.46}$&$84.92\pm2.05$&$103.78\pm\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.713\pm0.000$&\scriptsize$0.719\pm0.002$&\scriptsize$0.694\pm0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.21\pm\textbf{0.24}$&$\textbf{85.18}\pm\textbf{0.27}$&$108.18\pm0.73$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.503\pm0.006$&\scriptsize$0.536\pm0.026$&\scriptsize$0.511\pm0.016$\\
&$\rho_t=1$&metric&$\textbf{95.64}\pm0.40$&$83.41\pm2.36$&$109.33\pm0.71$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.955\pm0.038$&\scriptsize$0.997\pm0.014$&\scriptsize$1.000\pm0.018$\\
&none&metric&$95.09\pm1.13$&$83.69\pm2.41$&$\textbf{107.52}\pm\textbf{0.27}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.877\pm0.004$&\scriptsize$0.887\pm0.003$&\scriptsize$0.847\pm0.004$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$92.59\pm0.93$&\sout{$\textbf{82.01}\pm\textbf{3.21}$}&$\textbf{129.82}\pm\textbf{0.96}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.966\pm0.009$&\scriptsize\sout{$0.950\pm0.102$}&\scriptsize$0.978\pm0.208$\\
&none&metric&$\textbf{93.27}\pm\textbf{0.55}$&0&$130.18\pm1.06$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.248\pm0.033$&\scriptsize0&\scriptsize$1.690\pm0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\textbf{89.20}\pm\textbf{0.74}$&$\textbf{74.19}\pm\textbf{3.71}$&\sout{$\textbf{125.80}\pm\textbf{0.59}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999\pm0.001$&\scriptsize$1.000\pm0.000$&\scriptsize\sout{$0.876\pm0.176$}\\
&none&metric&$88.26\pm1.19$&$71.73\pm nan$&$128.19\pm~nan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.213\pm0.008$&\scriptsize$1.129\pm~nan$&\scriptsize$1.093\pm~nan$\\
\midrule\bottomrule
\end{tabular}
\caption{\textbf{Effect of stabilization across tasks and networks.} The network preparation by pre-training to stability, generally helps performance, with $\rho_t=0.5$ generally being preferable over $\rho_t=1$ across tasks and networks, with networks of depth $d=2$. Here we report the test set results across three different tasks. Metrics are accuracy for sl-MNIST and SHD, the higher the better, and perplexity for PTB, the lower the better. The non-differentiable networks, were often unable to reach a target norm of $\rho_t=0.5$, but the preparation to $\rho_t=1$ was still often beneficial. \red{ The strike through the number means that it wasn't close enough to the target radius, where close enough means at a distance of $0.05$, and those experiments are currently running again.}}
\label{tab:lsctask}
\end{table*}


% 11 -> 10
\begin{table}[]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN$\sigma$&$\rho_t=0.5$&metric&$11.19\pm~0.30$&$\textbf{14.71}\pm~3.50$&\sout{$643.26\pm~\textbf{0.70}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.498\pm~0.003$&\scriptsize$0.498\pm~0.002$&\scriptsize\sout{$0.202\pm~0.001$}\\
&$\rho_t=1$&metric&$11.45\pm~\textbf{0.20}$&$11.01\pm~\textbf{3.38}$&\sout{$\textbf{395.55}\pm~286.50$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.006\pm~0.017$&\scriptsize$1.012\pm~0.021$&\scriptsize\sout{$1.072\pm~0.112$}\\
&none&metric&$\textbf{11.51}\pm~0.21$&$12.90\pm~3.82$&$643.23\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.356\pm~0.001$&\scriptsize$0.361\pm~0.001$&\scriptsize$0.351\pm~0.001$\\
\midrule
RNN$ReLU$&$\rho_t=0.5$&metric&$17.15\pm~4.90$&$\textbf{24.90}\pm~3.62$&\sout{$515.00\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.505\pm~0.008$&\scriptsize$0.511\pm~0.003$&\scriptsize\sout{$0.427\pm~nan$}\\
&$\rho_t=1$&metric&$17.90\pm~\textbf{2.04}$&\sout{$18.73\pm~\textbf{1.73}$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.002\pm~0.006$&\scriptsize\sout{$0.859\pm~0.163$}&\scriptsize0\\
&none&metric&$\textbf{19.63}\pm~6.60$&$16.43\pm~3.51$&$\textbf{500.04}\pm~\textbf{94.49}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323\pm~0.009$&\scriptsize$1.341\pm~0.006$&\scriptsize$0.769\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\textbf{95.61}\pm~\textbf{0.28}$&$86.47\pm~\textbf{0.60}$&\sout{$652.90\pm~6.50$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.502\pm~0.002$&\scriptsize$0.500\pm~0.002$&\scriptsize\sout{$0.448\pm~0.002$}\\
&$\rho_t=1$&metric&$94.33\pm~1.31$&$86.44\pm~1.48$&\sout{$\textbf{113.00}\pm~\textbf{0.66}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999\pm~0.008$&\scriptsize$1.016\pm~0.017$&\scriptsize\sout{$0.919\pm~0.046$}\\
&none&metric&$\textbf{95.61}\pm~0.38$&$\textbf{88.17}\pm~1.70$&$650.56\pm~1.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695\pm~0.003$&\scriptsize$0.702\pm~0.001$&\scriptsize$0.686\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.90\pm~0.30$&$80.18\pm~2.41$&$642.86\pm~1.05$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.501\pm~0.001$&\scriptsize$0.506\pm~0.010$&\scriptsize$0.509\pm~0.002$\\
&$\rho_t=1$&metric&$53.70\pm~48.80$&$\textbf{84.53}\pm~\textbf{2.10}$&$\textbf{262.52}\pm~253.12$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.996\pm~0.006$&\scriptsize$1.010\pm~0.007$&\scriptsize$0.961\pm~0.054$\\
&none&metric&$\textbf{96.07}\pm~\textbf{0.17}$&$59.68\pm~38.46$&$644.18\pm~\textbf{0.59}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858\pm~0.002$&\scriptsize$0.872\pm~0.001$&\scriptsize$0.854\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$\textbf{46.93}\pm~41.49$}&$\textbf{39.44}\pm~\textbf{17.85}$&\sout{$\textbf{658.06}\pm~5.53$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.803\pm~0.008$}&\scriptsize$1.003\pm~0.005$&\scriptsize\sout{$0.620\pm~0.003$}\\
&none&metric&$11.22\pm~\textbf{0.10}$&0&$666.46\pm~\textbf{0.61}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.272\pm~0.014$&\scriptsize0&\scriptsize$1.657\pm~0.033$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$10.76\pm~0.80$&$35.64\pm~\textbf{17.13}$&\sout{$664.09\pm~3.06$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.990\pm~0.011$&\scriptsize$1.000\pm~0.001$&\scriptsize\sout{$0.619\pm~0.002$}\\
&none&metric&$\textbf{10.82}\pm~\textbf{0.68}$&$\textbf{37.21}\pm~nan$&$\textbf{661.75}\pm~\textbf{0.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.087\pm~0.007$&\scriptsize$0.980\pm~nan$&\scriptsize$0.973\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{Depth 5}
\label{tab:depth5}
\end{table}



\begin{table*}[!ht]
\centering
\addtolength{\leftskip} {-1cm}
\addtolength{\rightskip}{-1cm}
\resizebox{1.1\textwidth}{!}{%

% 9 -> 5
\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN$\sigma$&$\rho_t=0.5$&metric&$\textbf{41.29}\pm\textbf{3.82}$&$30.38\pm\textbf{6.97}$&$\textbf{14.71}\pm3.50$&$\textbf{7.99}\pm3.43$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504\pm0.005$&\scriptsize$0.500\pm0.003$&\scriptsize$0.498\pm0.002$&\scriptsize$0.500\pm0.002$\\
&$\rho_t=1$&metric&$38.50\pm4.71$&$27.99\pm11.55$&$11.01\pm\textbf{3.38}$&$4.94\pm0.16$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.992\pm0.016$&\scriptsize$1.019\pm0.077$&\scriptsize$1.012\pm0.021$&\scriptsize$1.003\pm0.004$\\
&none&metric&$38.20\pm6.84$&$\textbf{30.47}\pm13.34$&$12.90\pm3.82$&$5.06\pm\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366\pm0.001$&\scriptsize$0.362\pm0.001$&\scriptsize$0.361\pm0.001$&\scriptsize$0.361\pm0.000$\\
\midrule
RNN$ReLU$&$\rho_t=0.5$&metric&$37.48\pm9.97$&$26.52\pm6.23$&$\textbf{24.90}\pm3.62$&$\textbf{18.27}\pm2.88$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.512\pm0.003$&\scriptsize$0.511\pm0.003$&\scriptsize$0.511\pm0.003$&\scriptsize$0.512\pm0.001$\\
&$\rho_t=1$&metric&\sout{$34.03\pm\textbf{4.43}$}&$28.24\pm\textbf{5.18}$&\sout{$18.73\pm\textbf{1.73}$}&\sout{$15.78\pm5.05$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.821\pm0.199$}&\scriptsize$1.004\pm0.010$&\scriptsize\sout{$0.859\pm0.163$}&\scriptsize\sout{$0.731\pm0.007$}\\
&none&metric&$\textbf{39.06}\pm10.85$&$\textbf{34.19}\pm5.98$&$16.43\pm3.51$&$15.59\pm\textbf{2.31}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355\pm0.004$&\scriptsize$1.346\pm0.003$&\scriptsize$1.341\pm0.006$&\scriptsize$1.339\pm0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\textbf{85.95}\pm\textbf{1.15}$&$\textbf{86.05}\pm2.98$&$86.47\pm\textbf{0.60}$&$85.06\pm2.41$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.461\pm0.006$&\scriptsize$0.495\pm0.009$&\scriptsize$0.500\pm0.002$&\scriptsize$0.500\pm0.002$\\
&$\rho_t=1$&metric&$76.01\pm3.56$&$84.29\pm\textbf{1.79}$&$86.44\pm1.48$&$83.69\pm2.88$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.993\pm0.006$&\scriptsize$1.006\pm0.005$&\scriptsize$1.016\pm0.017$&\scriptsize$1.031\pm0.021$\\
&none&metric&$84.55\pm1.45$&$86.01\pm2.48$&$\textbf{88.17}\pm1.70$&$\textbf{85.10}\pm\textbf{1.39}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751\pm0.002$&\scriptsize$0.710\pm0.002$&\scriptsize$0.702\pm0.001$&\scriptsize$0.699\pm0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$\textbf{81.99}\pm\textbf{1.65}$&$\textbf{86.75}\pm\textbf{0.44}$&$80.18\pm2.41$&$62.16\pm38.41$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.528\pm0.006$&\scriptsize$0.514\pm0.014$&\scriptsize$0.506\pm0.010$&\scriptsize$0.504\pm0.003$\\
&$\rho_t=1$&metric&$66.73\pm25.41$&$84.15\pm1.81$&$\textbf{84.53}\pm\textbf{2.10}$&$\textbf{71.49}\pm26.49$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.978\pm0.032$&\scriptsize$1.005\pm0.007$&\scriptsize$1.010\pm0.007$&\scriptsize$1.030\pm0.028$\\
&none&metric&$76.69\pm9.27$&$84.98\pm3.17$&$59.68\pm38.46$&$24.28\pm\textbf{2.72}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914\pm0.003$&\scriptsize$0.879\pm0.002$&\scriptsize$0.872\pm0.001$&\scriptsize$0.868\pm0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$\textbf{78.10}\pm\textbf{1.24}$&$\textbf{74.34}\pm8.61$&$\textbf{39.44}\pm\textbf{17.85}$&$\textbf{5.55}\pm\textbf{1.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.003\pm0.005$&\scriptsize$1.008\pm0.035$&\scriptsize$1.003\pm0.005$&\scriptsize$0.969\pm0.047$\\
&none&metric&$76.94\pm2.06$&$74.01\pm\textbf{2.75}$&0&$4.28\pmnan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853\pm0.023$&\scriptsize$1.707\pm0.016$&\scriptsize0&\scriptsize$1.651\pmnan$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\textbf{67.74}\pm\textbf{1.52}$&$\textbf{74.60}\pm\textbf{2.55}$&$35.64\pm\textbf{17.13}$&$\textbf{9.69}\pm8.96$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.000\pm0.003$&\scriptsize$1.001\pm0.002$&\scriptsize$1.000\pm0.001$&\scriptsize$1.000\pm0.001$\\
&none&metric&$66.83\pm4.23$&0&$\textbf{37.21}\pmnan$&$4.88\pm\textbf{0.10}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460\pm0.007$&\scriptsize0&\scriptsize$0.980\pmnan$&\scriptsize$0.933\pm0.002$\\
\midrule\bottomrule
\end{tabular}
}
\caption{\textbf{Effect of stabilization across depths and networks.} Networks of different depths are trained on the SHD task. All seem to benefit of the stabilization technique used before training, and  especially when the networks are prepared to have a $\rho_t=0.5$ as the networks become deeper. }
\label{tab:lscdepth}
\end{table*}



\newpage
\clearpage
\section{ May 14}

\begin{table*}[h]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{29.38}~\pm~6.65$&$34.66~\pm~8.30$&$\cellcolor{NiceGreen!25}\textbf{116.81}~\pm~7.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.492~\pm~0.008$&\scriptsize$0.496~\pm~0.007$&\scriptsize$0.497~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$27.30~\pm~2.57$}&$37.00~\pm~\textbf{3.80}$&\sout{$149.32~\pm~20.17$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.878~\pm~0.166$}&\scriptsize$1.003~\pm~0.004$&\scriptsize\sout{$0.916~\pm~0.013$}\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{28.12}~\pm~3.41$&$35.46~\pm~10.64$&\sout{$159.84~\pm~7.27$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.508~\pm~0.003$&\scriptsize\sout{$0.414~\pm~0.001$}\\
&$\rho_t=1$&metric&$24.80~\pm~5.44$&\sout{$33.93~\pm~\textbf{4.96}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{159.65}~\pm~7.50$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.997~\pm~0.009$&\scriptsize\sout{$0.845~\pm~0.177$}&\scriptsize\sout{$0.414~\pm~0.001$}\\
&none&metric&$23.51~\pm~\textbf{2.50}$&$\textbf{39.84}~\pm~5.91$&$173.67~\pm~\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{95.43}~\pm~\textbf{0.39}$&$\cellcolor{NiceGreen!25}\textbf{85.58}~\pm~\textbf{1.35}$&$\cellcolor{NiceGreen!25}\textbf{103.12}~\pm~0.25$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.485~\pm~0.021$&\scriptsize$0.491~\pm~0.006$&\scriptsize$0.499~\pm~0.001$\\
&$\rho_t=1$&metric&$95.04~\pm~0.75$&$84.40~\pm~2.21$&$103.41~\pm~0.78$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.004$&\scriptsize$1.003~\pm~0.005$&\scriptsize$1.002~\pm~0.004$\\
&none&metric&$94.85~\pm~0.40$&$84.92~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.21~\pm~\textbf{0.24}$&\sout{$59.66~\pm~18.29$}&$\cellcolor{NiceGreen!25}\textbf{108.09}~\pm~0.86$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.503~\pm~0.006$&\scriptsize\sout{$0.536~\pm~0.031$}&\scriptsize$0.503~\pm~0.005$\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{95.31}~\pm~0.52$}&$83.59~\pm~2.86$&$108.99~\pm~\textbf{0.29}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.955~\pm~0.038$}&\scriptsize$1.004~\pm~0.004$&\scriptsize$1.009~\pm~0.004$\\
&none&metric&$95.21~\pm~0.95$&$\textbf{83.61}~\pm~\textbf{1.97}$&$108.93~\pm~2.83$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{92.77}~\pm~\textbf{0.57}$}&$\cellcolor{NiceOrange!25}\textbf{83.18}~\pm~\textbf{0.95}$&\sout{$141.39~\pm~12.27$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.967~\pm~0.015$}&\scriptsize$1.001~\pm~0.001$&\scriptsize\sout{$0.918~\pm~0.208$}\\
&none&metric&$86.38~\pm~5.16$&$70.26~\pm~7.12$&$\textbf{130.18}~\pm~\textbf{1.06}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.225~\pm~0.033$&\scriptsize$1.748~\pm~0.016$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{82.05}~\pm~6.26$&$\cellcolor{NiceOrange!25}\textbf{73.98}~\pm~\textbf{3.75}$&\sout{$158.54~\pm~26.89$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.001$&\scriptsize$1.000~\pm~0.000$&\scriptsize\sout{$0.735~\pm~0.075$}\\
&none&metric&$81.42~\pm~\textbf{1.17}$&$68.20~\pm~6.85$&$\textbf{133.18}~\pm~\textbf{7.05}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.212~\pm~0.007$&\scriptsize$1.130~\pm~0.003$&\scriptsize$1.094~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{\textbf{Effect of stabilization across tasks and networks.} The network preparation by pre-training to stability, generally helps performance, with $\rho_t=0.5$ generally being preferable over $\rho_t=1$ across tasks and networks, with networks of depth $d=2$. Here we report the test set results across three different tasks. Metrics are accuracy for sl-MNIST and SHD, the higher the better, and perplexity for PTB, the lower the better. The non-differentiable networks, were often unable to reach a target norm of $\rho_t=0.5$, but the preparation to $\rho_t=1$ was still often beneficial. \red{ The strike through the number means that it wasn't close enough to the target radius, where close enough means at a distance of $0.05$, and those experiments are currently running again.}}
\label{tab:lsctask}
\end{table*}


\begin{table}[h]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN$\sigma$&$\rho_t=0.5$&metric&$11.19~\pm~0.30$&$\textbf{14.71}~\pm~3.50$&\sout{$640.79~\pm~\textbf{0.14}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.498~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize\sout{$0.202~\pm~0.001$}\\
&$\rho_t=1$&metric&$\textbf{11.52}~\pm~\textbf{0.12}$&$12.21~\pm~\textbf{1.32}$&\sout{$\textbf{431.34}~\pm~242.13$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.991~\pm~0.010$&\scriptsize$1.009~\pm~0.017$&\scriptsize\sout{$0.938~\pm~0.122$}\\
&none&metric&$11.41~\pm~0.20$&$12.90~\pm~3.82$&$643.23~\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN$ReLU$&$\rho_t=0.5$&metric&$17.15~\pm~4.90$&$24.90~\pm~3.62$&\sout{$\textbf{176.87}~\pm~\textbf{36.19}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.505~\pm~0.008$&\scriptsize$0.511~\pm~0.003$&\scriptsize\sout{$0.427~\pm~0.002$}\\
&$\rho_t=1$&metric&$17.90~\pm~\textbf{2.04}$&\sout{$\textbf{25.87}~\pm~10.18$}&\sout{$178.60~\pm~42.65$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.002~\pm~0.006$&\scriptsize\sout{$0.859~\pm~0.163$}&\scriptsize\sout{$0.429~\pm~0.003$}\\
&none&metric&$\textbf{19.63}~\pm~6.60$&$16.43~\pm~\textbf{3.51}$&$500.04~\pm~94.49$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\textbf{95.61}~\pm~\textbf{0.28}$&$86.47~\pm~\textbf{0.60}$&\sout{$641.26~\pm~\textbf{0.11}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.502~\pm~0.002$&\scriptsize$0.500~\pm~0.002$&\scriptsize\sout{$0.447~\pm~0.001$}\\
&$\rho_t=1$&metric&$94.33~\pm~1.31$&$87.26~\pm~1.90$&\sout{$\textbf{134.87}~\pm~5.07$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.008$&\scriptsize$1.003~\pm~0.001$&\scriptsize\sout{$0.953~\pm~0.024$}\\
&none&metric&$\textbf{95.61}~\pm~0.38$&$\textbf{88.12}~\pm~1.39$&$648.25~\pm~4.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.92~\pm~0.31$&$\textbf{82.12}~\pm~\textbf{2.70}$&$642.86~\pm~1.05$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.501~\pm~0.001$&\scriptsize$0.506~\pm~0.008$&\scriptsize$0.509~\pm~0.002$\\
&$\rho_t=1$&metric&$53.70~\pm~48.80$&$81.34~\pm~6.23$&$\textbf{142.69}~\pm~11.78$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.996~\pm~0.006$&\scriptsize$1.010~\pm~0.007$&\scriptsize$0.985~\pm~0.083$\\
&none&metric&$\textbf{96.19}~\pm~\textbf{0.29}$&$62.98~\pm~27.77$&$644.18~\pm~\textbf{0.59}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$11.32~\pm~\textbf{0.23}$}&$\textbf{6.17}~\pm~1.86$&\sout{$\textbf{644.53}~\pm~\textbf{0.24}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.891~\pm~0.066$}&\scriptsize$1.000~\pm~0.007$&\scriptsize\sout{$0.620~\pm~0.003$}\\
&none&metric&$\textbf{11.75}~\pm~0.71$&$4.87~\pm~\textbf{0.11}$&$655.61~\pm~12.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.281~\pm~0.014$&\scriptsize$1.671~\pm~0.002$&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$10.76~\pm~\textbf{0.80}$&$\textbf{40.96}~\pm~20.69$&\sout{$\textbf{643.48}~\pm~\textbf{0.11}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.990~\pm~0.011$&\scriptsize$1.000~\pm~0.001$&\scriptsize\sout{$0.619~\pm~0.002$}\\
&none&metric&$\textbf{11.73}~\pm~1.54$&$19.84~\pm~\textbf{6.56}$&$661.75~\pm~0.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize$0.979~\pm~0.003$&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{Depth 5}
\label{tab:depth5}
\end{table}



\begin{table*}[!ht]
\centering
\addtolength{\leftskip} {-1cm}
\addtolength{\rightskip}{-1cm}
\resizebox{1.1\textwidth}{!}{%

% 9 -> 5
\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN$\sigma$&$\rho_t=0.5$&metric&$\textbf{41.29}~\pm~3.82$&$30.38~\pm~6.97$&$\textbf{14.71}~\pm~3.50$&$\textbf{7.99}~\pm~3.43$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.005$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize$0.500~\pm~0.002$\\
&$\rho_t=1$&metric&$36.63~\pm~\textbf{2.97}$&\sout{$15.31~\pm~\textbf{1.05}$}&$12.21~\pm~\textbf{1.32}$&$4.83~\pm~0.16$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.992~\pm~0.016$&\scriptsize\sout{$1.030~\pm~0.119$}&\scriptsize$1.009~\pm~0.017$&\scriptsize$1.003~\pm~0.004$\\
&none&metric&$38.20~\pm~6.84$&$\textbf{30.47}~\pm~13.34$&$12.90~\pm~3.82$&$5.06~\pm~\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN$ReLU$&$\rho_t=0.5$&metric&$37.48~\pm~9.97$&$26.52~\pm~6.23$&$24.90~\pm~3.62$&$18.27~\pm~2.88$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.512~\pm~0.003$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.512~\pm~0.001$\\
&$\rho_t=1$&metric&\sout{$36.79~\pm~\textbf{2.26}$}&$28.24~\pm~\textbf{5.18}$&\sout{$\textbf{25.87}~\pm~10.18$}&\sout{$\textbf{22.50}~\pm~4.38$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.821~\pm~0.199$}&\scriptsize$1.004~\pm~0.010$&\scriptsize\sout{$0.859~\pm~0.163$}&\scriptsize\sout{$0.731~\pm~0.007$}\\
&none&metric&$\textbf{39.06}~\pm~10.85$&$\textbf{34.19}~\pm~5.98$&$16.43~\pm~\textbf{3.51}$&$15.59~\pm~\textbf{2.31}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&\sout{$80.62~\pm~nan$}&$\textbf{86.05}~\pm~2.98$&$86.47~\pm~\textbf{0.60}$&$85.03~\pm~2.38$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.453~\pm~nan$}&\scriptsize$0.495~\pm~0.009$&\scriptsize$0.500~\pm~0.002$&\scriptsize$0.500~\pm~0.002$\\
&$\rho_t=1$&metric&$76.01~\pm~3.56$&$84.29~\pm~\textbf{1.79}$&$87.26~\pm~1.90$&\sout{$85.10~\pm~2.53$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.993~\pm~0.006$&\scriptsize$1.006~\pm~0.005$&\scriptsize$1.003~\pm~0.001$&\scriptsize\sout{$1.031~\pm~0.021$}\\
&none&metric&$\textbf{84.55}~\pm~\textbf{1.45}$&$86.01~\pm~2.48$&$\textbf{88.12}~\pm~1.39$&$\textbf{87.40}~\pm~\textbf{2.29}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.699~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$61.72~\pm~29.02$}&$\textbf{86.86}~\pm~\textbf{0.48}$&$\textbf{82.12}~\pm~\textbf{2.70}$&$43.71~\pm~44.85$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.532~\pm~0.003$}&\scriptsize$0.508~\pm~0.007$&\scriptsize$0.506~\pm~0.008$&\scriptsize$0.504~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$60.34~\pm~24.50$}&$84.15~\pm~1.81$&$81.34~\pm~6.23$&\sout{$\textbf{56.58}~\pm~24.22$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.978~\pm~0.032$}&\scriptsize$1.005~\pm~0.007$&\scriptsize$1.010~\pm~0.007$&\scriptsize\sout{$1.030~\pm~0.028$}\\
&none&metric&$\textbf{76.69}~\pm~\textbf{9.27}$&$83.74~\pm~2.81$&$62.98~\pm~27.77$&$27.90~\pm~\textbf{7.79}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.879~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$\textbf{78.10}~\pm~\textbf{1.24}$&$46.41~\pm~9.78$&$\textbf{6.17}~\pm~1.86$&$\textbf{5.59}~\pm~1.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.003~\pm~0.005$&\scriptsize$1.012~\pm~0.032$&\scriptsize$1.000~\pm~0.007$&\scriptsize$1.003~\pm~0.011$\\
&none&metric&$77.18~\pm~1.59$&$\textbf{57.88}~\pm~\textbf{6.96}$&$4.87~\pm~\textbf{0.11}$&$5.03~\pm~\textbf{0.11}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize$1.701~\pm~0.011$&\scriptsize$1.671~\pm~0.002$&\scriptsize$1.654~\pm~0.004$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\textbf{67.74}~\pm~\textbf{1.52}$&$\textbf{66.92}~\pm~\textbf{2.50}$&$\textbf{40.96}~\pm~20.69$&$\textbf{14.20}~\pm~6.21$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.000~\pm~0.003$&\scriptsize$1.001~\pm~0.002$&\scriptsize$1.000~\pm~0.001$&\scriptsize$1.000~\pm~0.000$\\
&none&metric&$66.83~\pm~4.23$&$60.47~\pm~7.05$&$19.84~\pm~\textbf{6.56}$&$5.06~\pm~\textbf{0.18}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize$1.016~\pm~0.001$&\scriptsize$0.979~\pm~0.003$&\scriptsize$0.933~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}
}
\caption{\textbf{Effect of stabilization across depths and networks.} Networks of different depths are trained on the SHD task. All seem to benefit of the stabilization technique used before training, and  especially when the networks are prepared to have a $\rho_t=0.5$ as the networks become deeper. }
\label{tab:lscdepth}
\end{table*}





\newpage
\clearpage
\section{May 19}


% 11 -> 8
\begin{table*}[h]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{29.38}~\pm~6.65$&$34.66~\pm~8.30$&$\cellcolor{NiceGreen!25}\textbf{127.97}~\pm~23.09$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.492~\pm~0.008$&\scriptsize$0.496~\pm~0.007$&\scriptsize$0.492~\pm~0.011$\\
&$\rho_t=1$&metric&\sout{$27.57~\pm~3.85$}&$32.75~\pm~\textbf{6.12}$&\sout{$145.06~\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.900~\pm~0.142$}&\scriptsize$1.019~\pm~0.019$&\scriptsize\sout{$0.939~\pm~nan$}\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{28.12}~\pm~3.41$&$35.46~\pm~10.64$&\sout{$\cellcolor{NiceGreen!25}\textbf{161.83}~\pm~8.83$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.508~\pm~0.003$&\scriptsize\sout{$0.414~\pm~0.001$}\\
&$\rho_t=1$&metric&$24.80~\pm~5.44$&\sout{$33.30~\pm~\textbf{4.89}$}&\sout{$162.02~\pm~8.94$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.997~\pm~0.009$&\scriptsize\sout{$0.845~\pm~0.177$}&\scriptsize\sout{$0.414~\pm~0.001$}\\
&none&metric&$23.51~\pm~\textbf{2.50}$&$\textbf{39.84}~\pm~5.91$&$173.67~\pm~\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{95.42}~\pm~\textbf{0.32}$}&$\cellcolor{NiceGreen!25}\textbf{85.58}~\pm~\textbf{1.35}$&$\cellcolor{NiceGreen!25}\textbf{103.12}~\pm~0.25$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.480~\pm~0.020$}&\scriptsize$0.491~\pm~0.006$&\scriptsize$0.499~\pm~0.001$\\
&$\rho_t=1$&metric&$95.04~\pm~0.75$&$84.40~\pm~2.21$&$103.41~\pm~0.78$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.004$&\scriptsize$1.003~\pm~0.005$&\scriptsize$1.002~\pm~0.004$\\
&none&metric&$94.85~\pm~0.40$&$84.92~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.21~\pm~\textbf{0.24}$&\sout{$64.29~\pm~24.40$}&$\cellcolor{NiceGreen!25}\textbf{108.09}~\pm~\textbf{0.86}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.503~\pm~0.006$&\scriptsize\sout{$0.536~\pm~0.026$}&\scriptsize$0.503~\pm~0.005$\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{95.46}~\pm~0.38$}&$82.87~\pm~2.75$&$109.93~\pm~1.90$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.955~\pm~0.038$}&\scriptsize$0.997~\pm~0.014$&\scriptsize$1.000~\pm~0.018$\\
&none&metric&$95.21~\pm~0.95$&$\textbf{83.61}~\pm~\textbf{1.97}$&$108.93~\pm~2.83$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{91.25}~\pm~\textbf{1.48}$}&$\cellcolor{NiceOrange!25}\textbf{83.18}~\pm~\textbf{0.95}$&\sout{$133.64~\pm~5.25$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.769~\pm~0.003$}&\scriptsize$1.001~\pm~0.001$&\scriptsize\sout{$0.846~\pm~0.222$}\\
&none&metric&$86.38~\pm~5.16$&$70.26~\pm~7.12$&$\textbf{130.18}~\pm~\textbf{1.06}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.225~\pm~0.033$&\scriptsize$1.748~\pm~0.016$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{82.05}~\pm~6.26$&$\cellcolor{NiceOrange!25}\textbf{73.98}~\pm~\textbf{3.75}$&\sout{$134.29~\pm~\textbf{1.44}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.001$&\scriptsize$1.000~\pm~0.000$&\scriptsize\sout{$0.687~\pm~0.005$}\\
&none&metric&$81.42~\pm~\textbf{1.17}$&$68.20~\pm~6.85$&$\textbf{130.54}~\pm~5.09$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.212~\pm~0.007$&\scriptsize$1.130~\pm~0.003$&\scriptsize$1.094~\pm~0.002$\\
\midrule\bottomrule
\end{tabular}

\caption{\textbf{Effect of stabilization across tasks and networks.} The network preparation by pre-training to stability, generally helps performance, with $\rho_t=0.5$ generally being preferable over $\rho_t=1$ across tasks and networks, with networks of depth $d=2$. Here we report the test set results across three different tasks. Metrics are accuracy for sl-MNIST and SHD, the higher the better ($\uparrow$), and perplexity for PTB, the lower the better ($\downarrow$). The non-differentiable networks, were often unable to reach a target norm of $\rho_t=0.5$, but the preparation to $\rho_t=1$ was still often beneficial. \red{ The strike through the number means that it wasn't close enough to the target radius, where close enough means at a distance of $0.05$, and those experiments are currently running again.}}
\label{tab:lsctask}
\end{table*}



% 11 -> 10
\begin{table}[h]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$11.19~\pm~0.30$&$\cellcolor{NiceGreen!25}\textbf{14.71}~\pm~3.50$&\sout{$640.79~\pm~\textbf{0.14}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.498~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize\sout{$0.202~\pm~0.001$}\\
&$\rho_t=1$&metric&$11.14~\pm~0.77$&$11.72~\pm~\textbf{1.46}$&\sout{$\cellcolor{NiceOrange!25}\textbf{538.82}~\pm~202.60$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.019$&\scriptsize$1.016~\pm~0.019$&\scriptsize\sout{$0.944~\pm~0.109$}\\
&none&metric&$\textbf{11.41}~\pm~\textbf{0.20}$&$12.90~\pm~3.82$&$643.23~\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$17.15~\pm~4.90$&$\cellcolor{NiceGreen!25}\textbf{24.90}~\pm~3.62$&$644.26~\pm~\textbf{1.71}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.505~\pm~0.008$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.501~\pm~0.003$\\
&$\rho_t=1$&metric&$17.90~\pm~\textbf{2.04}$&\sout{$20.93~\pm~\textbf{1.56}$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.002~\pm~0.006$&\scriptsize\sout{$0.859~\pm~0.163$}&\scriptsize0\\
&none&metric&$\textbf{19.63}~\pm~6.60$&$16.43~\pm~3.51$&$\textbf{500.04}~\pm~94.49$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{95.61}~\pm~\textbf{0.28}$&$86.47~\pm~\textbf{0.60}$&\sout{$641.27~\pm~\textbf{0.10}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.502~\pm~0.002$&\scriptsize$0.500~\pm~0.002$&\scriptsize\sout{$0.448~\pm~0.002$}\\
&$\rho_t=1$&metric&$94.33~\pm~1.31$&$86.73~\pm~1.42$&\sout{$\cellcolor{NiceOrange!25}\textbf{126.16}~\pm~6.97$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.008$&\scriptsize$1.016~\pm~0.017$&\scriptsize\sout{$0.962~\pm~0.020$}\\
&none&metric&$\textbf{95.61}~\pm~0.38$&$\textbf{88.12}~\pm~1.39$&$648.25~\pm~4.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.92~\pm~0.31$&$\cellcolor{NiceGreen!25}\textbf{82.12}~\pm~\textbf{2.70}$&$642.86~\pm~1.05$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.501~\pm~0.001$&\scriptsize$0.506~\pm~0.008$&\scriptsize$0.509~\pm~0.002$\\
&$\rho_t=1$&metric&$53.70~\pm~48.80$&$80.17~\pm~8.50$&\sout{$\cellcolor{NiceOrange!25}\textbf{263.29}~\pm~251.11$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.996~\pm~0.006$&\scriptsize$1.010~\pm~0.007$&\scriptsize\sout{$0.954~\pm~0.060$}\\
&none&metric&$\textbf{96.19}~\pm~\textbf{0.29}$&$62.98~\pm~27.77$&$644.18~\pm~\textbf{0.59}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$11.30~\pm~\textbf{0.13}$}&$\cellcolor{NiceOrange!25}\textbf{6.17}~\pm~1.86$&\sout{$\cellcolor{NiceOrange!25}\textbf{644.53}~\pm~\textbf{0.26}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.753~\pm~0.001$}&\scriptsize$1.000~\pm~0.007$&\scriptsize\sout{$0.621~\pm~0.003$}\\
&none&metric&$\textbf{11.75}~\pm~0.71$&$4.93~\pm~\textbf{0.14}$&$655.61~\pm~12.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.281~\pm~0.014$&\scriptsize$1.667~\pm~0.007$&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$10.76~\pm~\textbf{0.80}$&$\cellcolor{NiceOrange!25}\textbf{40.96}~\pm~20.69$&\sout{$\cellcolor{NiceOrange!25}\textbf{643.45}~\pm~\textbf{0.11}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.990~\pm~0.011$&\scriptsize$1.000~\pm~0.001$&\scriptsize\sout{$0.621~\pm~0.003$}\\
&none&metric&$\textbf{11.73}~\pm~1.54$&$18.89~\pm~\textbf{5.68}$&$661.75~\pm~0.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}


\caption{Depth 5}
\label{tab:depth5}
\end{table}



\begin{table*}[!ht]
\centering
\addtolength{\leftskip} {-1cm}
\addtolength{\rightskip}{-1cm}
\resizebox{1.1\textwidth}{!}{%

% 9 -> 5

\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{41.29}~\pm~\textbf{3.82}$&$30.38~\pm~\textbf{6.97}$&$\cellcolor{NiceGreen!25}\textbf{14.71}~\pm~3.50$&$\cellcolor{NiceGreen!25}\textbf{7.99}~\pm~3.43$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.005$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize$0.500~\pm~0.002$\\
&$\rho_t=1$&metric&$37.94~\pm~3.91$&$22.72~\pm~8.04$&$11.72~\pm~\textbf{1.46}$&$4.83~\pm~0.16$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.992~\pm~0.016$&\scriptsize$1.019~\pm~0.077$&\scriptsize$1.016~\pm~0.019$&\scriptsize$1.003~\pm~0.004$\\
&none&metric&$38.20~\pm~6.84$&$\textbf{30.47}~\pm~13.34$&$12.90~\pm~3.82$&$5.06~\pm~\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN$ReLU$&$\rho_t=0.5$&metric&$37.48~\pm~9.97$&$26.52~\pm~6.23$&$\cellcolor{NiceGreen!25}\textbf{24.90}~\pm~3.62$&$18.27~\pm~2.88$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.512~\pm~0.003$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.512~\pm~0.001$\\
&$\rho_t=1$&metric&\sout{$36.28~\pm~\textbf{3.28}$}&$28.24~\pm~\textbf{5.18}$&\sout{$20.93~\pm~\textbf{1.56}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{21.88}~\pm~4.96$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.821~\pm~0.199$}&\scriptsize$1.004~\pm~0.010$&\scriptsize\sout{$0.859~\pm~0.163$}&\scriptsize\sout{$0.731~\pm~0.007$}\\
&none&metric&$\textbf{39.06}~\pm~10.85$&$\textbf{34.19}~\pm~5.98$&$16.43~\pm~3.51$&$15.59~\pm~\textbf{2.31}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&\sout{$81.27~\pm~1.81$}&$\cellcolor{NiceGreen!25}\textbf{86.05}~\pm~2.98$&$86.47~\pm~\textbf{0.60}$&$85.03~\pm~2.38$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.461~\pm~0.006$}&\scriptsize$0.495~\pm~0.009$&\scriptsize$0.500~\pm~0.002$&\scriptsize$0.500~\pm~0.002$\\
&$\rho_t=1$&metric&$76.01~\pm~3.56$&$84.29~\pm~\textbf{1.79}$&$86.73~\pm~1.42$&\sout{$85.73~\pm~\textbf{1.72}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.993~\pm~0.006$&\scriptsize$1.006~\pm~0.005$&\scriptsize$1.016~\pm~0.017$&\scriptsize\sout{$1.031~\pm~0.021$}\\
&none&metric&$\textbf{84.55}~\pm~\textbf{1.45}$&$86.01~\pm~2.48$&$\textbf{88.12}~\pm~1.39$&$\textbf{87.40}~\pm~2.29$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.699~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$42.52~\pm~\textbf{7.18}$}&$\cellcolor{NiceGreen!25}\textbf{87.14}~\pm~\textbf{0.69}$&$\cellcolor{NiceGreen!25}\textbf{82.12}~\pm~\textbf{2.70}$&$43.71~\pm~44.85$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.528~\pm~0.006$}&\scriptsize$0.514~\pm~0.014$&\scriptsize$0.506~\pm~0.008$&\scriptsize$0.504~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$67.39~\pm~25.89$}&$84.15~\pm~1.81$&$80.17~\pm~8.50$&\sout{$\cellcolor{NiceOrange!25}\textbf{56.80}~\pm~25.30$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.978~\pm~0.032$}&\scriptsize$1.005~\pm~0.007$&\scriptsize$1.010~\pm~0.007$&\scriptsize\sout{$1.030~\pm~0.028$}\\
&none&metric&$\textbf{76.69}~\pm~9.27$&$83.74~\pm~2.81$&$62.98~\pm~27.77$&$27.90~\pm~\textbf{7.79}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.879~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{78.10}~\pm~\textbf{1.24}$&\sout{$52.33~\pm~18.36$}&$\cellcolor{NiceOrange!25}\textbf{6.17}~\pm~1.86$&$\cellcolor{NiceOrange!25}\textbf{5.59}~\pm~1.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.003~\pm~0.005$&\scriptsize\sout{$0.932~\pm~0.129$}&\scriptsize$1.000~\pm~0.007$&\scriptsize$1.003~\pm~0.011$\\
&none&metric&$77.18~\pm~1.59$&$\textbf{57.88}~\pm~\textbf{6.96}$&$4.93~\pm~\textbf{0.14}$&$4.93~\pm~\textbf{0.23}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize$1.701~\pm~0.011$&\scriptsize$1.667~\pm~0.007$&\scriptsize$1.656~\pm~0.005$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{67.74}~\pm~\textbf{1.52}$&$\cellcolor{NiceOrange!25}\textbf{66.92}~\pm~\textbf{2.50}$&$\cellcolor{NiceOrange!25}\textbf{40.96}~\pm~20.69$&\sout{$\cellcolor{NiceOrange!25}\textbf{11.96}~\pm~6.76$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.000~\pm~0.003$&\scriptsize$1.001~\pm~0.002$&\scriptsize$1.000~\pm~0.001$&\scriptsize\sout{$0.917~\pm~0.166$}\\
&none&metric&$66.83~\pm~4.23$&$60.47~\pm~7.05$&$18.89~\pm~\textbf{5.68}$&$5.06~\pm~\textbf{0.18}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize$1.016~\pm~0.001$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.933~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

}
\caption{\textbf{Effect of stabilization across depths and networks.} Networks of different depths are trained on the SHD task. All seem to benefit of the stabilization technique used before training, and  especially when the networks are prepared to have a $\rho_t=0.5$ as the networks become deeper. }
\label{tab:lscdepth}
\end{table*}




\newpage
\clearpage
\section{May 21}

% 11 -> 8
\begin{table*}[h]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{29.38}~\pm~6.65$&$34.66~\pm~8.30$&$\cellcolor{NiceGreen!25}\textbf{116.81}~\pm~7.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.492~\pm~0.008$&\scriptsize$0.496~\pm~0.007$&\scriptsize$0.497~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$26.39~\pm~\textbf{1.49}$}&$35.10~\pm~\textbf{7.45}$&\sout{$395.35~\pm~285.28$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.900~\pm~0.142$}&\scriptsize$1.019~\pm~0.019$&\scriptsize\sout{$0.574~\pm~0.409$}\\
&none&metric&$29.02~\pm~2.00$&$\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{28.12}~\pm~3.41$&$35.46~\pm~10.64$&\sout{$\cellcolor{NiceGreen!25}\textbf{156.57}~\pm~6.95$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.508~\pm~0.003$&\scriptsize\sout{$0.415~\pm~0.002$}\\
&$\rho_t=1$&metric&$24.80~\pm~5.44$&\sout{$34.59~\pm~\textbf{5.35}$}&\sout{$162.79~\pm~15.62$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.997~\pm~0.009$&\scriptsize\sout{$0.845~\pm~0.177$}&\scriptsize\sout{$0.430~\pm~0.004$}\\
&none&metric&$23.51~\pm~\textbf{2.50}$&$\textbf{39.84}~\pm~5.91$&$173.67~\pm~\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{95.28}~\pm~\textbf{0.17}$}&$\cellcolor{NiceGreen!25}\textbf{85.58}~\pm~\textbf{1.35}$&$\cellcolor{NiceGreen!25}\textbf{103.12}~\pm~0.25$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.480~\pm~0.020$}&\scriptsize$0.491~\pm~0.006$&\scriptsize$0.499~\pm~0.001$\\
&$\rho_t=1$&metric&$95.04~\pm~0.75$&$84.40~\pm~2.21$&$103.41~\pm~0.78$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.004$&\scriptsize$1.003~\pm~0.005$&\scriptsize$1.002~\pm~0.004$\\
&none&metric&$94.85~\pm~0.40$&$84.92~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.21~\pm~\textbf{0.24}$&\sout{$76.46~\pm~16.26$}&$109.01~\pm~\textbf{1.97}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.503~\pm~0.006$&\scriptsize\sout{$0.536~\pm~0.026$}&\scriptsize$0.511~\pm~0.016$\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{95.55}~\pm~0.45$}&$\cellcolor{NiceOrange!25}\textbf{83.77}~\pm~2.36$&$110.08~\pm~2.19$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.955~\pm~0.038$}&\scriptsize$0.997~\pm~0.014$&\scriptsize$1.000~\pm~0.018$\\
&none&metric&$95.21~\pm~0.95$&$83.61~\pm~\textbf{1.97}$&$\textbf{108.93}~\pm~2.83$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{89.12}~\pm~5.42$}&$\cellcolor{NiceOrange!25}\textbf{83.18}~\pm~\textbf{0.95}$&\sout{$143.20~\pm~12.42$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.776~\pm~0.009$}&\scriptsize$1.001~\pm~0.001$&\scriptsize\sout{$0.792~\pm~0.183$}\\
&none&metric&$86.38~\pm~\textbf{5.16}$&$70.26~\pm~7.12$&$\textbf{130.18}~\pm~\textbf{1.06}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.225~\pm~0.033$&\scriptsize$1.748~\pm~0.016$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{82.05}~\pm~6.26$&$\cellcolor{NiceOrange!25}\textbf{73.98}~\pm~\textbf{3.75}$&\sout{$138.79~\pm~\textbf{1.02}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.001$&\scriptsize$1.000~\pm~0.000$&\scriptsize\sout{$0.686~\pm~0.004$}\\
&none&metric&$81.42~\pm~\textbf{1.17}$&$68.20~\pm~6.85$&$\textbf{130.54}~\pm~5.09$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.212~\pm~0.007$&\scriptsize$1.130~\pm~0.003$&\scriptsize$1.094~\pm~0.002$\\
\midrule\bottomrule
\end{tabular}

\caption{\textbf{Effect of stabilization across tasks and networks.} The network preparation by pre-training to stability, generally helps performance, with $\rho_t=0.5$ generally being preferable over $\rho_t=1$ across tasks and networks, with networks of depth $d=2$. Here we report the test set results across three different tasks. Metrics are accuracy for sl-MNIST and SHD, the higher the better ($\uparrow$), and perplexity for PTB, the lower the better ($\downarrow$). The non-differentiable networks, were often unable to reach a target norm of $\rho_t=0.5$, but the preparation to $\rho_t=1$ was still often beneficial. \red{ The strike through the number means that it wasn't close enough to the target radius, where close enough means at a distance of $0.05$, and those experiments are currently running again.}}
\label{tab:lsctask}
\end{table*}


% 11 -> 10
\begin{table}[h]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$11.19~\pm~0.30$&$14.71~\pm~\textbf{3.50}$&\sout{$640.79~\pm~\textbf{0.14}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.498~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize\sout{$0.201~\pm~0.001$}\\
&$\rho_t=1$&metric&$11.14~\pm~0.77$&$\cellcolor{NiceOrange!25}\textbf{15.36}~\pm~3.66$&$\cellcolor{NiceOrange!25}\textbf{545.41}~\pm~189.42$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.019$&\scriptsize$1.016~\pm~0.019$&\scriptsize$0.998~\pm~0.073$\\
&none&metric&$\textbf{11.41}~\pm~\textbf{0.20}$&$12.90~\pm~3.82$&$643.23~\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$17.15~\pm~4.90$&$\cellcolor{NiceGreen!25}\textbf{24.90}~\pm~3.62$&$644.26~\pm~\textbf{1.71}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.505~\pm~0.008$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.501~\pm~0.003$\\
&$\rho_t=1$&metric&$17.90~\pm~\textbf{2.04}$&\sout{$21.82~\pm~\textbf{3.11}$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.002~\pm~0.006$&\scriptsize\sout{$0.859~\pm~0.163$}&\scriptsize0\\
&none&metric&$\textbf{19.63}~\pm~6.60$&$16.43~\pm~3.51$&$\textbf{500.04}~\pm~94.49$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{95.61}~\pm~\textbf{0.28}$&$86.47~\pm~\textbf{0.60}$&\sout{$641.27~\pm~\textbf{0.10}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.502~\pm~0.002$&\scriptsize$0.500~\pm~0.002$&\scriptsize\sout{$0.448~\pm~0.002$}\\
&$\rho_t=1$&metric&$94.33~\pm~1.31$&$87.10~\pm~1.12$&$\cellcolor{NiceOrange!25}\textbf{130.28}~\pm~19.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.008$&\scriptsize$1.016~\pm~0.017$&\scriptsize$0.983~\pm~0.018$\\
&none&metric&$\textbf{95.61}~\pm~0.38$&$\textbf{88.12}~\pm~1.39$&$648.25~\pm~4.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.92~\pm~0.31$&$82.12~\pm~2.70$&$642.86~\pm~1.05$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.501~\pm~0.001$&\scriptsize$0.506~\pm~0.008$&\scriptsize$0.509~\pm~0.002$\\
&$\rho_t=1$&metric&$53.70~\pm~48.80$&$\cellcolor{NiceOrange!25}\textbf{83.64}~\pm~\textbf{2.21}$&$\cellcolor{NiceOrange!25}\textbf{264.89}~\pm~250.24$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.996~\pm~0.006$&\scriptsize$1.010~\pm~0.007$&\scriptsize$0.985~\pm~0.035$\\
&none&metric&$\textbf{96.19}~\pm~\textbf{0.29}$&$62.98~\pm~27.77$&$644.18~\pm~\textbf{0.59}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$11.26~\pm~\textbf{0.10}$}&$\cellcolor{NiceOrange!25}\textbf{6.17}~\pm~1.86$&\sout{$\cellcolor{NiceOrange!25}\textbf{644.51}~\pm~\textbf{0.31}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.747~\pm~0.035$}&\scriptsize$1.000~\pm~0.007$&\scriptsize\sout{$0.621~\pm~0.003$}\\
&none&metric&$\textbf{11.75}~\pm~0.71$&$4.93~\pm~\textbf{0.14}$&$655.61~\pm~12.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.281~\pm~0.014$&\scriptsize$1.667~\pm~0.007$&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$10.76~\pm~\textbf{0.80}$&$\cellcolor{NiceOrange!25}\textbf{40.96}~\pm~20.69$&\sout{$\cellcolor{NiceOrange!25}\textbf{643.48}~\pm~\textbf{0.11}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.990~\pm~0.011$&\scriptsize$1.000~\pm~0.001$&\scriptsize\sout{$0.620~\pm~0.003$}\\
&none&metric&$\textbf{11.73}~\pm~1.54$&$18.89~\pm~\textbf{5.68}$&$661.75~\pm~0.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}


\caption{Depth 5}
\label{tab:depth5}
\end{table}



\begin{table*}[!ht]
\centering
\addtolength{\leftskip} {-1cm}
\addtolength{\rightskip}{-1cm}
\resizebox{1.1\textwidth}{!}{%
\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{41.29}~\pm~\textbf{3.82}$&$30.38~\pm~\textbf{6.97}$&$14.71~\pm~\textbf{3.50}$&$\cellcolor{NiceGreen!25}\textbf{7.99}~\pm~3.43$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.005$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize$0.500~\pm~0.002$\\
&$\rho_t=1$&metric&$37.96~\pm~3.93$&$20.87~\pm~7.19$&$\cellcolor{NiceOrange!25}\textbf{15.36}~\pm~3.66$&$4.83~\pm~0.16$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.992~\pm~0.016$&\scriptsize$1.019~\pm~0.077$&\scriptsize$1.016~\pm~0.019$&\scriptsize$1.003~\pm~0.004$\\
&none&metric&$38.20~\pm~6.84$&$\textbf{30.47}~\pm~13.34$&$12.90~\pm~3.82$&$5.06~\pm~\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$37.48~\pm~9.97$&$26.52~\pm~6.23$&$\cellcolor{NiceGreen!25}\textbf{24.90}~\pm~3.62$&$18.27~\pm~2.88$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.512~\pm~0.003$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.512~\pm~0.001$\\
&$\rho_t=1$&metric&\sout{$36.79~\pm~\textbf{2.26}$}&$28.24~\pm~\textbf{5.18}$&\sout{$21.82~\pm~\textbf{3.11}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{19.74}~\pm~7.30$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.821~\pm~0.199$}&\scriptsize$1.004~\pm~0.010$&\scriptsize\sout{$0.859~\pm~0.163$}&\scriptsize\sout{$0.731~\pm~0.007$}\\
&none&metric&$\textbf{39.06}~\pm~10.85$&$\textbf{34.19}~\pm~5.98$&$16.43~\pm~3.51$&$15.59~\pm~\textbf{2.31}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&\sout{$80.95~\pm~2.78$}&$\cellcolor{NiceGreen!25}\textbf{86.05}~\pm~2.98$&$86.47~\pm~\textbf{0.60}$&$85.03~\pm~2.38$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.461~\pm~0.006$}&\scriptsize$0.495~\pm~0.009$&\scriptsize$0.500~\pm~0.002$&\scriptsize$0.500~\pm~0.002$\\
&$\rho_t=1$&metric&$76.01~\pm~3.56$&$84.29~\pm~\textbf{1.79}$&$87.10~\pm~1.12$&\sout{$85.73~\pm~\textbf{1.72}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.993~\pm~0.006$&\scriptsize$1.006~\pm~0.005$&\scriptsize$1.016~\pm~0.017$&\scriptsize\sout{$1.031~\pm~0.021$}\\
&none&metric&$\textbf{84.55}~\pm~\textbf{1.45}$&$86.01~\pm~2.48$&$\textbf{88.12}~\pm~1.39$&$\textbf{87.40}~\pm~2.29$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.699~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$42.58~\pm~\textbf{1.69}$}&$\cellcolor{NiceGreen!25}\textbf{87.14}~\pm~\textbf{0.69}$&$82.12~\pm~2.70$&$43.71~\pm~44.85$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.528~\pm~0.006$}&\scriptsize$0.514~\pm~0.014$&\scriptsize$0.506~\pm~0.008$&\scriptsize$0.504~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$59.35~\pm~24.95$}&$84.15~\pm~1.81$&$\cellcolor{NiceOrange!25}\textbf{83.64}~\pm~\textbf{2.21}$&\sout{$\cellcolor{NiceOrange!25}\textbf{57.91}~\pm~24.69$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.978~\pm~0.032$}&\scriptsize$1.005~\pm~0.007$&\scriptsize$1.010~\pm~0.007$&\scriptsize\sout{$1.030~\pm~0.028$}\\
&none&metric&$\textbf{76.69}~\pm~9.27$&$83.74~\pm~2.81$&$62.98~\pm~27.77$&$27.90~\pm~\textbf{7.79}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.879~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{78.10}~\pm~\textbf{1.24}$&\sout{$52.38~\pm~18.44$}&$\cellcolor{NiceOrange!25}\textbf{6.17}~\pm~1.86$&$\cellcolor{NiceOrange!25}\textbf{5.59}~\pm~1.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.003~\pm~0.005$&\scriptsize\sout{$0.932~\pm~0.129$}&\scriptsize$1.000~\pm~0.007$&\scriptsize$1.003~\pm~0.011$\\
&none&metric&$77.18~\pm~1.59$&$\textbf{57.88}~\pm~\textbf{6.96}$&$4.93~\pm~\textbf{0.14}$&$4.93~\pm~\textbf{0.23}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize$1.701~\pm~0.011$&\scriptsize$1.667~\pm~0.007$&\scriptsize$1.656~\pm~0.005$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{67.74}~\pm~\textbf{1.52}$&$\cellcolor{NiceOrange!25}\textbf{66.92}~\pm~\textbf{2.50}$&$\cellcolor{NiceOrange!25}\textbf{40.96}~\pm~20.69$&\sout{$\cellcolor{NiceOrange!25}\textbf{11.96}~\pm~6.76$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.000~\pm~0.003$&\scriptsize$1.001~\pm~0.002$&\scriptsize$1.000~\pm~0.001$&\scriptsize\sout{$0.917~\pm~0.166$}\\
&none&metric&$66.83~\pm~4.23$&$60.47~\pm~7.05$&$18.89~\pm~\textbf{5.68}$&$5.06~\pm~\textbf{0.18}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize$1.016~\pm~0.001$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.933~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}
}
\caption{\textbf{Effect of stabilization across depths and networks.} Networks of different depths are trained on the SHD task. All seem to benefit of the stabilization technique used before training, and  especially when the networks are prepared to have a $\rho_t=0.5$ as the networks become deeper. }
\label{tab:lscdepth}
\end{table*}





\newpage
\clearpage
\section{June 1}


% 11 -> 8
\begin{table*}[h]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{29.38}~\pm~6.65$&$34.66~\pm~8.30$&$\cellcolor{NiceGreen!25}\textbf{116.81}~\pm~7.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.492~\pm~0.008$&\scriptsize$0.496~\pm~0.007$&\scriptsize$0.497~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$26.98~\pm~3.29$}&$36.37~\pm~\textbf{5.23}$&\sout{$276.09~\pm~244.64$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.900~\pm~0.142$}&\scriptsize$1.019~\pm~0.019$&\scriptsize\sout{$0.671~\pm~0.335$}\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{28.12}~\pm~3.41$&$35.46~\pm~10.64$&\sout{$\cellcolor{NiceGreen!25}\textbf{158.79}~\pm~10.43$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.508~\pm~0.003$&\scriptsize\sout{$0.416~\pm~0.002$}\\
&$\rho_t=1$&metric&$24.80~\pm~5.44$&\sout{$33.34~\pm~\textbf{4.90}$}&\sout{$167.83~\pm~13.57$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.997~\pm~0.009$&\scriptsize\sout{$0.845~\pm~0.177$}&\scriptsize\sout{$0.430~\pm~0.004$}\\
&none&metric&$23.51~\pm~\textbf{2.50}$&$\textbf{39.84}~\pm~5.91$&$173.67~\pm~\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{95.28}~\pm~\textbf{0.17}$}&$\cellcolor{NiceGreen!25}\textbf{85.58}~\pm~\textbf{1.35}$&$\cellcolor{NiceGreen!25}\textbf{103.12}~\pm~0.25$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.480~\pm~0.020$}&\scriptsize$0.491~\pm~0.006$&\scriptsize$0.499~\pm~0.001$\\
&$\rho_t=1$&metric&$95.04~\pm~0.75$&$84.40~\pm~2.21$&$103.41~\pm~0.78$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.004$&\scriptsize$1.003~\pm~0.005$&\scriptsize$1.002~\pm~0.004$\\
&none&metric&$94.85~\pm~0.40$&$84.92~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.21~\pm~\textbf{0.24}$&\sout{$66.83~\pm~20.71$}&$109.22~\pm~2.37$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.503~\pm~0.006$&\scriptsize\sout{$0.536~\pm~0.026$}&\scriptsize$0.511~\pm~0.016$\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{95.60}~\pm~0.40$}&$82.87~\pm~2.75$&$109.93~\pm~\textbf{1.90}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.955~\pm~0.038$}&\scriptsize$0.997~\pm~0.014$&\scriptsize$1.000~\pm~0.018$\\
&none&metric&$95.21~\pm~0.95$&$\textbf{83.61}~\pm~\textbf{1.97}$&$\textbf{108.93}~\pm~2.83$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{86.45}~\pm~\textbf{3.30}$}&$\cellcolor{NiceOrange!25}\textbf{83.18}~\pm~\textbf{0.95}$&\sout{$139.21~\pm~13.13$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.768~\pm~0.003$}&\scriptsize$1.001~\pm~0.001$&\scriptsize\sout{$0.899~\pm~0.148$}\\
&none&metric&$86.38~\pm~5.16$&$70.26~\pm~7.12$&$\textbf{130.18}~\pm~\textbf{1.06}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.225~\pm~0.033$&\scriptsize$1.748~\pm~0.016$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{82.05}~\pm~6.26$&$\cellcolor{NiceOrange!25}\textbf{73.98}~\pm~\textbf{3.75}$&\sout{$138.80~\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.001$&\scriptsize$1.000~\pm~0.000$&\scriptsize\sout{$0.691~\pm~nan$}\\
&none&metric&$81.42~\pm~\textbf{1.17}$&$68.20~\pm~6.85$&$\textbf{130.54}~\pm~\textbf{5.09}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.212~\pm~0.007$&\scriptsize$1.130~\pm~0.003$&\scriptsize$1.094~\pm~0.002$\\
\midrule\bottomrule
\end{tabular}

\caption{\textbf{Effect of stabilization across tasks and networks.} The network preparation by pre-training to stability, generally helps performance, with $\rho_t=0.5$ generally being preferable over $\rho_t=1$ across tasks and networks, with networks of depth $d=2$. Here we report the test set results across three different tasks. Metrics are accuracy for sl-MNIST and SHD, the higher the better ($\uparrow$), and perplexity for PTB, the lower the better ($\downarrow$). The non-differentiable networks, were often unable to reach a target norm of $\rho_t=0.5$, but the preparation to $\rho_t=1$ was still often beneficial. \red{ The strike through the number means that it wasn't close enough to the target radius, where close enough means at a distance of $0.05$, and those experiments are currently running again.}}
\label{tab:lsctask}
\end{table*}



% 11 -> 10
\begin{table}[h]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$11.19~\pm~0.30$&$\cellcolor{NiceGreen!25}\textbf{14.71}~\pm~\textbf{3.50}$&\sout{$640.79~\pm~\textbf{0.14}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.498~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize\sout{$0.201~\pm~0.001$}\\
&$\rho_t=1$&metric&$11.14~\pm~0.77$&$14.21~\pm~4.50$&$\cellcolor{NiceOrange!25}\textbf{536.77}~\pm~206.68$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.019$&\scriptsize$1.016~\pm~0.019$&\scriptsize$0.998~\pm~0.073$\\
&none&metric&$\textbf{11.41}~\pm~\textbf{0.20}$&$12.90~\pm~3.82$&$643.23~\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$17.15~\pm~4.90$&$\cellcolor{NiceGreen!25}\textbf{24.90}~\pm~3.62$&$644.26~\pm~\textbf{1.71}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.505~\pm~0.008$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.501~\pm~0.003$\\
&$\rho_t=1$&metric&$17.90~\pm~\textbf{2.04}$&\sout{$23.54~\pm~5.61$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.002~\pm~0.006$&\scriptsize\sout{$0.859~\pm~0.163$}&\scriptsize0\\
&none&metric&$\textbf{19.63}~\pm~6.60$&$16.43~\pm~\textbf{3.51}$&$\textbf{500.04}~\pm~94.49$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{95.61}~\pm~\textbf{0.28}$&$86.47~\pm~\textbf{0.60}$&\sout{$641.27~\pm~\textbf{0.10}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.502~\pm~0.002$&\scriptsize$0.500~\pm~0.002$&\scriptsize\sout{$0.448~\pm~0.002$}\\
&$\rho_t=1$&metric&$94.33~\pm~1.31$&$86.55~\pm~2.16$&$\cellcolor{NiceOrange!25}\textbf{129.92}~\pm~13.24$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.008$&\scriptsize$1.016~\pm~0.017$&\scriptsize$0.983~\pm~0.018$\\
&none&metric&$\textbf{95.61}~\pm~0.38$&$\textbf{88.12}~\pm~1.39$&$648.25~\pm~4.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.92~\pm~0.31$&$82.12~\pm~2.70$&$642.86~\pm~1.05$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.501~\pm~0.001$&\scriptsize$0.506~\pm~0.008$&\scriptsize$0.509~\pm~0.002$\\
&$\rho_t=1$&metric&$53.70~\pm~48.80$&$\cellcolor{NiceOrange!25}\textbf{84.51}~\pm~\textbf{1.77}$&$\cellcolor{NiceOrange!25}\textbf{267.78}~\pm~248.18$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.996~\pm~0.006$&\scriptsize$1.010~\pm~0.007$&\scriptsize$0.985~\pm~0.035$\\
&none&metric&$\textbf{96.19}~\pm~\textbf{0.29}$&$62.98~\pm~27.77$&$644.18~\pm~\textbf{0.59}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$11.43~\pm~\textbf{0.21}$}&$\cellcolor{NiceOrange!25}\textbf{6.17}~\pm~1.86$&\sout{$\cellcolor{NiceOrange!25}\textbf{645.99}~\pm~\textbf{0.82}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.754~\pm~0.002$}&\scriptsize$1.000~\pm~0.007$&\scriptsize\sout{$0.963~\pm~0.029$}\\
&none&metric&$\textbf{11.75}~\pm~0.71$&$4.93~\pm~\textbf{0.14}$&$655.61~\pm~12.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.281~\pm~0.014$&\scriptsize$1.667~\pm~0.007$&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$10.76~\pm~\textbf{0.80}$&$\cellcolor{NiceOrange!25}\textbf{40.96}~\pm~20.69$&\sout{$\cellcolor{NiceOrange!25}\textbf{642.95}~\pm~\textbf{0.37}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.990~\pm~0.011$&\scriptsize$1.000~\pm~0.001$&\scriptsize\sout{$0.676~\pm~0.010$}\\
&none&metric&$\textbf{11.73}~\pm~1.54$&$18.89~\pm~\textbf{5.68}$&$661.75~\pm~0.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}


\caption{Depth 5}
\label{tab:depth5}
\end{table}



\begin{table*}[!ht]
\centering
\addtolength{\leftskip} {-1cm}
\addtolength{\rightskip}{-1cm}
\resizebox{1.1\textwidth}{!}{%

\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{41.29}~\pm~\textbf{3.82}$&$30.38~\pm~\textbf{6.97}$&$\cellcolor{NiceGreen!25}\textbf{14.71}~\pm~\textbf{3.50}$&$\cellcolor{NiceGreen!25}\textbf{7.99}~\pm~3.43$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.005$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize$0.500~\pm~0.002$\\
&$\rho_t=1$&metric&$37.96~\pm~3.93$&$23.16~\pm~8.02$&$14.21~\pm~4.50$&$4.83~\pm~0.16$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.992~\pm~0.016$&\scriptsize$1.019~\pm~0.077$&\scriptsize$1.016~\pm~0.019$&\scriptsize$1.003~\pm~0.004$\\
&none&metric&$38.20~\pm~6.84$&$\textbf{30.47}~\pm~13.34$&$12.90~\pm~3.82$&$5.06~\pm~\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$37.48~\pm~9.97$&$26.52~\pm~6.23$&$\cellcolor{NiceGreen!25}\textbf{24.90}~\pm~3.62$&$18.27~\pm~2.88$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.512~\pm~0.003$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.511~\pm~0.003$&\scriptsize$0.512~\pm~0.001$\\
&$\rho_t=1$&metric&\sout{$35.68~\pm~\textbf{2.22}$}&$28.24~\pm~\textbf{5.18}$&\sout{$23.54~\pm~5.61$}&\sout{$\cellcolor{NiceOrange!25}\textbf{19.01}~\pm~\textbf{2.04}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.821~\pm~0.199$}&\scriptsize$1.004~\pm~0.010$&\scriptsize\sout{$0.859~\pm~0.163$}&\scriptsize\sout{$0.731~\pm~0.007$}\\
&none&metric&$\textbf{39.06}~\pm~10.85$&$\textbf{34.19}~\pm~5.98$&$16.43~\pm~\textbf{3.51}$&$15.59~\pm~2.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&\sout{$81.51~\pm~1.56$}&$\cellcolor{NiceGreen!25}\textbf{86.05}~\pm~2.98$&$86.47~\pm~\textbf{0.60}$&$85.03~\pm~2.38$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.461~\pm~0.006$}&\scriptsize$0.495~\pm~0.009$&\scriptsize$0.500~\pm~0.002$&\scriptsize$0.500~\pm~0.002$\\
&$\rho_t=1$&metric&$76.01~\pm~3.56$&$84.29~\pm~\textbf{1.79}$&$86.55~\pm~2.16$&\sout{$85.81~\pm~\textbf{1.74}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.993~\pm~0.006$&\scriptsize$1.006~\pm~0.005$&\scriptsize$1.016~\pm~0.017$&\scriptsize\sout{$1.031~\pm~0.021$}\\
&none&metric&$\textbf{84.55}~\pm~\textbf{1.45}$&$86.01~\pm~2.48$&$\textbf{88.12}~\pm~1.39$&$\textbf{87.40}~\pm~2.29$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.699~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$50.44~\pm~21.78$}&$\cellcolor{NiceGreen!25}\textbf{86.75}~\pm~\textbf{0.44}$&$82.12~\pm~2.70$&$43.71~\pm~44.85$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.528~\pm~0.006$}&\scriptsize$0.514~\pm~0.014$&\scriptsize$0.506~\pm~0.008$&\scriptsize$0.504~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$55.03~\pm~20.35$}&$84.15~\pm~1.81$&$\cellcolor{NiceOrange!25}\textbf{84.51}~\pm~\textbf{1.77}$&\sout{$\cellcolor{NiceOrange!25}\textbf{66.24}~\pm~24.62$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.978~\pm~0.032$}&\scriptsize$1.005~\pm~0.007$&\scriptsize$1.010~\pm~0.007$&\scriptsize\sout{$1.030~\pm~0.028$}\\
&none&metric&$\textbf{76.69}~\pm~\textbf{9.27}$&$83.74~\pm~2.81$&$62.98~\pm~27.77$&$27.90~\pm~\textbf{7.79}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.879~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{78.10}~\pm~\textbf{1.24}$&\sout{$45.72~\pm~9.27$}&$\cellcolor{NiceOrange!25}\textbf{6.17}~\pm~1.86$&$\cellcolor{NiceOrange!25}\textbf{5.59}~\pm~1.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.003~\pm~0.005$&\scriptsize\sout{$0.932~\pm~0.129$}&\scriptsize$1.000~\pm~0.007$&\scriptsize$1.003~\pm~0.011$\\
&none&metric&$77.18~\pm~1.59$&$\textbf{57.88}~\pm~\textbf{6.96}$&$4.93~\pm~\textbf{0.14}$&$4.93~\pm~\textbf{0.23}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize$1.701~\pm~0.011$&\scriptsize$1.667~\pm~0.007$&\scriptsize$1.656~\pm~0.005$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{67.74}~\pm~\textbf{1.52}$&$\cellcolor{NiceOrange!25}\textbf{66.92}~\pm~\textbf{2.50}$&$\cellcolor{NiceOrange!25}\textbf{40.96}~\pm~20.69$&\sout{$\cellcolor{NiceOrange!25}\textbf{11.96}~\pm~6.76$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.000~\pm~0.003$&\scriptsize$1.001~\pm~0.002$&\scriptsize$1.000~\pm~0.001$&\scriptsize\sout{$0.917~\pm~0.166$}\\
&none&metric&$66.83~\pm~4.23$&$60.47~\pm~7.05$&$18.89~\pm~\textbf{5.68}$&$5.06~\pm~\textbf{0.18}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize$1.016~\pm~0.001$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.933~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

}
\caption{\textbf{Effect of stabilization across depths and networks.} Networks of different depths are trained on the SHD task. All seem to benefit of the stabilization technique used before training, and  especially when the networks are prepared to have a $\rho_t=0.5$ as the networks become deeper. }
\label{tab:lscdepth}
\end{table*}


\newpage
\clearpage
\section{23 June 2023}

\begin{table}[]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{35.15}~\pm~7.92$}&\sout{$38.67~\pm~\textbf{5.19}$}&\sout{$\cellcolor{NiceGreen!25}\textbf{137.09}~\pm~31.40$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.530~\pm~0.017$}&\scriptsize\sout{$0.422~\pm~0.068$}&\scriptsize\sout{$0.348~\pm~0.119$}\\
&$\rho_t=1$&metric&\sout{$21.75~\pm~8.29$}&\sout{$18.49~\pm~13.33$}&\sout{$49421654336997193357983744.00~\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.090~\pm~0.136$}&\scriptsize\sout{$1.585~\pm~0.816$}&\scriptsize\sout{$1.305~\pm~nan$}\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\cellcolor{NiceBlue!25}\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{40.37}~\pm~8.51$}&$33.80~\pm~5.96$&\sout{$186.85~\pm~102.26$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.541~\pm~0.020$}&\scriptsize$0.500~\pm~0.004$&\scriptsize\sout{$0.474~\pm~0.011$}\\
&$\rho_t=1$&metric&\sout{$29.06~\pm~3.84$}&\sout{$26.69~\pm~\textbf{5.69}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{125.23}~\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.031~\pm~0.036$}&\scriptsize\sout{$1.064~\pm~0.091$}&\scriptsize\sout{$0.930~\pm~nan$}\\
&none&metric&$23.51~\pm~\textbf{2.50}$&$\cellcolor{NiceBlue!25}\textbf{39.84}~\pm~5.91$&$173.67~\pm~\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&$95.22~\pm~\textbf{0.21}$&$84.09~\pm~\textbf{0.97}$&$\cellcolor{NiceGreen!25}\textbf{100.28}~\pm~nan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.505~\pm~0.015$&\scriptsize$0.505~\pm~0.012$&\scriptsize$0.502~\pm~nan$\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{95.40}~\pm~0.80$}&\sout{$77.87~\pm~7.69$}&\sout{$101.77~\pm~2.51$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.382~\pm~0.436$}&\scriptsize\sout{$1.071~\pm~0.040$}&\scriptsize\sout{$0.978~\pm~0.047$}\\
&none&metric&$94.85~\pm~0.40$&$\cellcolor{NiceBlue!25}\textbf{84.92}~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$74.67~\pm~42.45$}&$59.41~\pm~23.88$&$\cellcolor{NiceGreen!25}\textbf{108.16}~\pm~\textbf{1.77}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.525~\pm~0.014$}&\scriptsize$0.499~\pm~0.001$&\scriptsize$0.510~\pm~0.005$\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{95.49}~\pm~\textbf{0.91}$}&\sout{$60.54~\pm~31.37$}&\sout{$109.63~\pm~2.00$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.169~\pm~0.178$}&\scriptsize\sout{$1.134~\pm~0.075$}&\scriptsize\sout{$1.082~\pm~0.025$}\\
&none&metric&$95.21~\pm~0.95$&$\cellcolor{NiceBlue!25}\textbf{83.61}~\pm~\textbf{1.97}$&$108.93~\pm~2.83$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$61.72~\pm~43.90$}&\sout{$67.85~\pm~7.14$}&$647.18~\pm~\textbf{0.96}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.970~\pm~0.050$}&\scriptsize\sout{$0.923~\pm~0.109$}&\scriptsize$0.994~\pm~0.056$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{86.38}~\pm~\textbf{5.16}$&$\cellcolor{NiceBlue!25}\textbf{70.26}~\pm~\textbf{7.12}$&$\cellcolor{NiceBlue!25}\textbf{130.18}~\pm~1.06$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.225~\pm~0.033$&\scriptsize$1.748~\pm~0.016$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&0&$\cellcolor{NiceOrange!25}\textbf{75.55}~\pm~\textbf{0.50}$&\sout{$645.09~\pm~\textbf{1.94}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize$1.000~\pm~0.004$&\scriptsize\sout{$1.044~\pm~0.031$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{81.42}~\pm~\textbf{1.17}$&$68.20~\pm~6.85$&$\cellcolor{NiceBlue!25}\textbf{130.54}~\pm~5.09$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.212~\pm~0.007$&\scriptsize$1.130~\pm~0.003$&\scriptsize$1.094~\pm~0.002$\\
\midrule\bottomrule
\end{tabular}

\end{table}

\begin{table}[]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$11.32~\pm~0.24$&$\cellcolor{NiceGreen!25}\textbf{14.57}~\pm~6.05$&\sout{$\cellcolor{NiceGreen!25}\textbf{638.74}~\pm~\textbf{0.40}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.491~\pm~0.021$&\scriptsize\sout{$0.532~\pm~0.051$}\\
&$\rho_t=1$&metric&\sout{$11.18~\pm~1.22$}&\sout{$8.41~\pm~4.46$}&\sout{$659.35~\pm~36.27$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.978~\pm~0.034$}&\scriptsize\sout{$1.121~\pm~0.192$}&\scriptsize\sout{$0.978~\pm~0.044$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.41}~\pm~\textbf{0.20}$&$12.90~\pm~\textbf{3.82}$&$643.23~\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{31.56}~\pm~7.05$&$\cellcolor{NiceGreen!25}\textbf{20.96}~\pm~6.33$&\sout{$623.75~\pm~\textbf{75.35}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.516~\pm~0.023$&\scriptsize$0.516~\pm~0.014$&\scriptsize\sout{$0.480~\pm~0.012$}\\
&$\rho_t=1$&metric&0&\sout{$20.34~\pm~nan$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize\sout{$1.026~\pm~nan$}&\scriptsize0\\
&none&metric&$19.63~\pm~\textbf{6.60}$&$16.43~\pm~\textbf{3.51}$&$\cellcolor{NiceBlue!25}\textbf{500.04}~\pm~94.49$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{96.67}~\pm~\textbf{0.33}$&$83.99~\pm~nan$&\sout{$\cellcolor{NiceGreen!25}\textbf{256.58}~\pm~256.28$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.506~\pm~0.007$&\scriptsize$0.506~\pm~nan$&\scriptsize\sout{$0.523~\pm~0.034$}\\
&$\rho_t=1$&metric&\sout{$80.69~\pm~32.30$}&\sout{$70.63~\pm~nan$}&\sout{$644.32~\pm~\textbf{0.40}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.179~\pm~0.138$}&\scriptsize\sout{$1.092~\pm~nan$}&\scriptsize\sout{$1.098~\pm~0.047$}\\
&none&metric&$95.61~\pm~0.38$&$\cellcolor{NiceBlue!25}\textbf{88.12}~\pm~\textbf{1.39}$&$648.25~\pm~4.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$68.26~\pm~49.60$&\sout{$43.51~\pm~54.73$}&\sout{$639.90~\pm~\textbf{0.22}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.503~\pm~0.002$&\scriptsize\sout{$0.536~\pm~0.021$}&\scriptsize\sout{$0.553~\pm~0.089$}\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{96.24}~\pm~\textbf{0.22}$}&\sout{$62.68~\pm~\textbf{25.56}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{158.37}~\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.173~\pm~0.165$}&\scriptsize\sout{$1.129~\pm~0.081$}&\scriptsize\sout{$1.152~\pm~nan$}\\
&none&metric&$96.19~\pm~0.29$&$\cellcolor{NiceBlue!25}\textbf{62.98}~\pm~27.77$&$644.18~\pm~0.59$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$11.33~\pm~\textbf{0.25}$}&$\cellcolor{NiceOrange!25}\textbf{5.00}~\pm~0.17$&\sout{$\cellcolor{NiceOrange!25}\textbf{649.52}~\pm~\textbf{0.95}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.978~\pm~0.079$}&\scriptsize$0.993~\pm~0.027$&\scriptsize\sout{$0.958~\pm~0.057$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.75}~\pm~0.71$&$4.93~\pm~\textbf{0.14}$&$655.61~\pm~12.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.281~\pm~0.014$&\scriptsize$1.667~\pm~0.007$&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$10.83~\pm~\textbf{0.63}$&$\cellcolor{NiceOrange!25}\textbf{43.03}~\pm~12.65$&$\cellcolor{NiceOrange!25}\textbf{650.16}~\pm~\textbf{0.39}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.008$&\scriptsize$0.996~\pm~0.001$&\scriptsize$0.999~\pm~0.066$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.73}~\pm~1.54$&$18.89~\pm~\textbf{5.68}$&$661.75~\pm~0.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\end{table}

\begin{table}[]
\centering
\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{40.32}~\pm~\textbf{5.29}$&$\cellcolor{NiceGreen!25}\textbf{39.18}~\pm~\textbf{4.30}$&$\cellcolor{NiceGreen!25}\textbf{14.57}~\pm~6.05$&$4.79~\pm~\textbf{0.15}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.513~\pm~0.021$&\scriptsize$0.506~\pm~0.019$&\scriptsize$0.491~\pm~0.021$&\scriptsize$0.483~\pm~0.002$\\
&$\rho_t=1$&metric&\sout{$35.00~\pm~8.87$}&\sout{$23.38~\pm~12.35$}&\sout{$8.41~\pm~4.46$}&\sout{$\cellcolor{NiceOrange!25}\textbf{5.31}~\pm~0.77$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.297~\pm~0.122$}&\scriptsize\sout{$1.230~\pm~0.389$}&\scriptsize\sout{$1.121~\pm~0.192$}&\scriptsize\sout{$1.044~\pm~0.009$}\\
&none&metric&$38.20~\pm~6.84$&$30.47~\pm~13.34$&$12.90~\pm~\textbf{3.82}$&$5.06~\pm~0.16$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$29.60~\pm~\textbf{6.66}$&$31.29~\pm~6.87$&$\cellcolor{NiceGreen!25}\textbf{20.96}~\pm~6.33$&\sout{$\cellcolor{NiceGreen!25}\textbf{16.06}~\pm~\textbf{1.71}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.499~\pm~0.004$&\scriptsize$0.516~\pm~0.014$&\scriptsize\sout{$0.549~\pm~0.023$}\\
&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{39.17}~\pm~10.89$&\sout{$\cellcolor{NiceOrange!25}\textbf{36.60}~\pm~7.94$}&\sout{$20.34~\pm~nan$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.991~\pm~0.018$&\scriptsize\sout{$1.025~\pm~0.044$}&\scriptsize\sout{$1.026~\pm~nan$}&\scriptsize0\\
&none&metric&$39.06~\pm~10.85$&$34.19~\pm~\textbf{5.98}$&$16.43~\pm~\textbf{3.51}$&$15.59~\pm~2.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&$81.39~\pm~3.19$&$85.81~\pm~\textbf{1.13}$&$83.99~\pm~nan$&$\cellcolor{NiceGreen!25}\textbf{87.48}~\pm~\textbf{0.78}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.490~\pm~0.010$&\scriptsize$0.497~\pm~0.003$&\scriptsize$0.506~\pm~nan$&\scriptsize$0.502~\pm~0.002$\\
&$\rho_t=1$&metric&$66.53~\pm~6.34$&\sout{$79.63~\pm~6.00$}&\sout{$70.63~\pm~nan$}&\sout{$46.47~\pm~58.17$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.006~\pm~0.016$&\scriptsize\sout{$1.067~\pm~0.055$}&\scriptsize\sout{$1.092~\pm~nan$}&\scriptsize\sout{$1.167~\pm~0.132$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{84.55}~\pm~\textbf{1.45}$&$\cellcolor{NiceBlue!25}\textbf{86.01}~\pm~2.48$&$\cellcolor{NiceBlue!25}\textbf{88.12}~\pm~\textbf{1.39}$&$87.40~\pm~2.29$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.702~\pm~0.002$&\scriptsize$0.699~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$70.84~\pm~17.19$}&\sout{$24.40~\pm~14.58$}&\sout{$43.51~\pm~54.73$}&\sout{$21.70~\pm~28.71$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.603~\pm~0.090$}&\scriptsize\sout{$0.535~\pm~0.014$}&\scriptsize\sout{$0.536~\pm~0.021$}&\scriptsize\sout{$0.532~\pm~0.018$}\\
&$\rho_t=1$&metric&$44.44~\pm~\textbf{3.70}$&\sout{$82.38~\pm~\textbf{2.07}$}&\sout{$62.68~\pm~\textbf{25.56}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{52.04}~\pm~41.83$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.013~\pm~0.026$&\scriptsize\sout{$1.282~\pm~0.007$}&\scriptsize\sout{$1.129~\pm~0.081$}&\scriptsize\sout{$1.083~\pm~0.128$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{76.69}~\pm~9.27$&$\cellcolor{NiceBlue!25}\textbf{83.74}~\pm~2.81$&$\cellcolor{NiceBlue!25}\textbf{62.98}~\pm~27.77$&$27.90~\pm~\textbf{7.79}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.879~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$76.53~\pm~\textbf{0.76}$&\sout{$51.50~\pm~23.97$}&$\cellcolor{NiceOrange!25}\textbf{5.00}~\pm~0.17$&\sout{$\cellcolor{NiceOrange!25}\textbf{5.05}~\pm~\textbf{0.14}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.005~\pm~0.011$&\scriptsize\sout{$0.972~\pm~0.013$}&\scriptsize$0.993~\pm~0.027$&\scriptsize\sout{$0.980~\pm~0.017$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{77.18}~\pm~1.59$&$\cellcolor{NiceBlue!25}\textbf{57.88}~\pm~\textbf{6.96}$&$4.93~\pm~\textbf{0.14}$&$4.93~\pm~0.23$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize$1.701~\pm~0.011$&\scriptsize$1.667~\pm~0.007$&\scriptsize$1.656~\pm~0.005$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$66.81~\pm~\textbf{3.82}$&\sout{$18.85~\pm~nan$}&$\cellcolor{NiceOrange!25}\textbf{43.03}~\pm~12.65$&$4.92~\pm~\textbf{0.10}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.002~\pm~0.003$&\scriptsize\sout{$1.038~\pm~nan$}&\scriptsize$0.996~\pm~0.001$&\scriptsize$1.008~\pm~0.018$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{66.83}~\pm~4.23$&$\cellcolor{NiceBlue!25}\textbf{60.47}~\pm~\textbf{7.05}$&$18.89~\pm~\textbf{5.68}$&$\cellcolor{NiceBlue!25}\textbf{5.06}~\pm~0.18$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize$1.016~\pm~0.001$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.933~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\end{table}




\newpage
\clearpage
\section{June 28}



\begin{table}[]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{36.73}~\pm~8.86$}&\sout{$37.39~\pm~\textbf{5.31}$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.532~\pm~0.046$}&\scriptsize\sout{$1.321~\pm~0.584$}&\scriptsize0\\
&$\rho_t=1$&metric&\sout{$22.26~\pm~7.12$}&\sout{$17.18~\pm~6.25$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$2.203~\pm~1.072$}&\scriptsize\sout{$3.753~\pm~2.642$}&\scriptsize0\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\cellcolor{NiceBlue!25}\textbf{46.40}~\pm~12.12$&$\cellcolor{NiceBlue!25}\textbf{641.65}~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{34.16}~\pm~7.12$}&$33.80~\pm~5.96$&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.534~\pm~0.027$}&\scriptsize$0.500~\pm~0.004$&\scriptsize0\\
&$\rho_t=1$&metric&\sout{$32.18~\pm~\textbf{1.59}$}&$30.71~\pm~nan$&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.039~\pm~0.062$}&\scriptsize$0.999~\pm~nan$&\scriptsize0\\
&none&metric&$23.51~\pm~2.50$&$\cellcolor{NiceBlue!25}\textbf{39.84}~\pm~\textbf{5.91}$&$\cellcolor{NiceBlue!25}\textbf{173.67}~\pm~\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{95.35}~\pm~\textbf{0.23}$&$84.29~\pm~\textbf{1.28}$&$\cellcolor{NiceGreen!25}\textbf{100.28}~\pm~nan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.516~\pm~0.019$&\scriptsize$0.501~\pm~0.009$&\scriptsize$0.502~\pm~nan$\\
&$\rho_t=1$&metric&\sout{$94.13~\pm~2.40$}&\sout{$74.15~\pm~nan$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.621~\pm~0.957$}&\scriptsize\sout{$1.104~\pm~nan$}&\scriptsize0\\
&none&metric&$94.85~\pm~0.40$&$\cellcolor{NiceBlue!25}\textbf{84.92}~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$67.24~\pm~48.71$}&$52.14~\pm~23.19$&$110.56~\pm~nan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.530~\pm~0.018$}&\scriptsize$0.499~\pm~0.001$&\scriptsize$0.505~\pm~nan$\\
&$\rho_t=1$&metric&\sout{$83.06~\pm~24.34$}&\sout{$45.67~\pm~26.11$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.302~\pm~0.198$}&\scriptsize\sout{$1.071~\pm~0.041$}&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{95.13}~\pm~\textbf{0.93}$&$\cellcolor{NiceBlue!25}\textbf{83.61}~\pm~\textbf{1.97}$&$\cellcolor{NiceBlue!25}\textbf{107.52}~\pm~\textbf{0.27}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.004$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&0&0&\sout{$649.26~\pm~\textbf{0.32}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize0&\scriptsize\sout{$2.921~\pm~0.336$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{92.88}~\pm~nan$&$\cellcolor{NiceBlue!25}\textbf{74.89}~\pm~nan$&$\cellcolor{NiceBlue!25}\textbf{130.18}~\pm~1.06$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.225~\pm~nan$&\scriptsize$1.740~\pm~nan$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&0&$\cellcolor{NiceOrange!25}\textbf{75.28}~\pm~nan$&\sout{$645.23~\pm~\textbf{1.29}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize$0.996~\pm~nan$&\scriptsize\sout{$2.185~\pm~0.311$}\\
&none&metric&0&0&$\cellcolor{NiceBlue!25}\textbf{128.19}~\pm~nan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize0&\scriptsize$1.093~\pm~nan$\\
\midrule\bottomrule
\end{tabular}

\end{table}


\begin{table}[]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$11.32~\pm~\textbf{0.24}$&\sout{$\cellcolor{NiceGreen!25}\textbf{12.98}~\pm~1.70$}&\sout{$638.61~\pm~0.21$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.005$&\scriptsize\sout{$0.638~\pm~0.033$}&\scriptsize\sout{$0.633~\pm~0.201$}\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{11.50}~\pm~2.17$}&\sout{$4.69~\pm~\textbf{0.10}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{638.24}~\pm~\textbf{0.11}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.529~\pm~0.218$}&\scriptsize\sout{$1.669~\pm~0.501$}&\scriptsize\sout{$1.430~\pm~0.117$}\\
&none&metric&$11.37~\pm~0.27$&$12.90~\pm~3.82$&$643.23~\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{31.84}~\pm~6.68$}&\sout{$\cellcolor{NiceGreen!25}\textbf{22.14}~\pm~12.37$}&\sout{$518.76~\pm~132.43$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.542~\pm~0.035$}&\scriptsize\sout{$0.547~\pm~0.040$}&\scriptsize\sout{$0.434~\pm~0.045$}\\
&$\rho_t=1$&metric&\sout{$25.12~\pm~nan$}&\sout{$17.69~\pm~\textbf{1.29}$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.975~\pm~nan$}&\scriptsize\sout{$1.041~\pm~0.014$}&\scriptsize0\\
&none&metric&$19.63~\pm~\textbf{6.60}$&$16.43~\pm~3.51$&$\cellcolor{NiceBlue!25}\textbf{500.04}~\pm~\textbf{94.49}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{96.53}~\pm~\textbf{0.21}$&0&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.510~\pm~0.003$&\scriptsize0&\scriptsize0\\
&$\rho_t=1$&metric&\sout{$70.87~\pm~44.87$}&0&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.156~\pm~0.187$}&\scriptsize0&\scriptsize0\\
&none&metric&$95.61~\pm~0.38$&$\cellcolor{NiceBlue!25}\textbf{88.17}~\pm~\textbf{1.70}$&$\cellcolor{NiceBlue!25}\textbf{648.25}~\pm~\textbf{4.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.702~\pm~0.001$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$75.12~\pm~42.76$&\sout{$4.81~\pm~nan$}&$\cellcolor{NiceGreen!25}\textbf{640.17}~\pm~\textbf{0.37}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.509~\pm~0.009$&\scriptsize\sout{$0.535~\pm~nan$}&\scriptsize$0.517~\pm~0.017$\\
&$\rho_t=1$&metric&\sout{$95.83~\pm~\textbf{0.03}$}&0&\sout{$640.22~\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.029~\pm~0.079$}&\scriptsize0&\scriptsize\sout{$1.873~\pm~nan$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{96.19}~\pm~0.29$&$\cellcolor{NiceBlue!25}\textbf{62.98}~\pm~\textbf{27.77}$&$644.18~\pm~0.59$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&0&\sout{$\cellcolor{NiceOrange!25}\textbf{5.05}~\pm~nan$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize\sout{$1.024~\pm~nan$}&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.22}~\pm~\textbf{0.10}$&0&$\cellcolor{NiceBlue!25}\textbf{655.61}~\pm~\textbf{12.53}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.272~\pm~0.014$&\scriptsize0&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&0&0&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize0&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.73}~\pm~\textbf{1.54}$&0&$\cellcolor{NiceBlue!25}\textbf{661.75}~\pm~\textbf{0.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize0&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{task:5}
\end{table}



\begin{table}[]
\centering
\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{40.49}~\pm~5.91$}&\sout{$\cellcolor{NiceGreen!25}\textbf{31.18}~\pm~\textbf{4.80}$}&\sout{$\cellcolor{NiceGreen!25}\textbf{12.98}~\pm~1.70$}&\sout{$4.76~\pm~0.20$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.716~\pm~0.193$}&\scriptsize\sout{$1.229~\pm~0.675$}&\scriptsize\sout{$0.638~\pm~0.033$}&\scriptsize\sout{$0.858~\pm~0.533$}\\
&$\rho_t=1$&metric&\sout{$36.92~\pm~\textbf{4.81}$}&\sout{$18.22~\pm~8.23$}&\sout{$4.69~\pm~\textbf{0.10}$}&\sout{$4.78~\pm~0.24$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$5.843~\pm~4.956$}&\scriptsize\sout{$1.717~\pm~0.405$}&\scriptsize\sout{$1.669~\pm~0.501$}&\scriptsize\sout{$1.443~\pm~0.052$}\\
&none&metric&$38.20~\pm~6.84$&$30.47~\pm~13.34$&$12.90~\pm~3.82$&$\cellcolor{NiceBlue!25}\textbf{5.06}~\pm~\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$35.00~\pm~\textbf{8.56}$&$31.71~\pm~6.72$&\sout{$\cellcolor{NiceGreen!25}\textbf{22.14}~\pm~12.37$}&\sout{$12.53~\pm~\textbf{2.23}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.511~\pm~0.028$&\scriptsize\sout{$0.547~\pm~0.040$}&\scriptsize\sout{$0.612~\pm~0.016$}\\
&$\rho_t=1$&metric&$34.83~\pm~11.24$&$\cellcolor{NiceOrange!25}\textbf{41.15}~\pm~\textbf{1.36}$&\sout{$17.69~\pm~\textbf{1.29}$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.011~\pm~0.040$&\scriptsize$0.999~\pm~0.002$&\scriptsize\sout{$1.041~\pm~0.014$}&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{39.06}~\pm~10.85$&$34.19~\pm~5.98$&$16.43~\pm~3.51$&$\cellcolor{NiceBlue!25}\textbf{15.59}~\pm~2.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&$75.10~\pm~10.53$&$\cellcolor{NiceGreen!25}\textbf{86.04}~\pm~\textbf{1.25}$&0&$\cellcolor{NiceGreen!25}\textbf{87.55}~\pm~nan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.489~\pm~0.015$&\scriptsize$0.496~\pm~0.004$&\scriptsize0&\scriptsize$0.502~\pm~nan$\\
&$\rho_t=1$&metric&\sout{$69.64~\pm~3.92$}&0&0&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.043~\pm~0.077$}&\scriptsize0&\scriptsize0&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{84.55}~\pm~\textbf{1.45}$&$86.01~\pm~2.48$&$\cellcolor{NiceBlue!25}\textbf{88.17}~\pm~\textbf{1.70}$&$85.96~\pm~\textbf{0.61}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.702~\pm~0.001$&\scriptsize$0.700~\pm~0.001$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$68.37~\pm~15.23$}&$46.01~\pm~nan$&\sout{$4.81~\pm~nan$}&\sout{$5.29~\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.551~\pm~0.059$}&\scriptsize$0.508~\pm~nan$&\scriptsize\sout{$0.535~\pm~nan$}&\scriptsize\sout{$0.549~\pm~nan$}\\
&$\rho_t=1$&metric&$41.98~\pm~\textbf{4.08}$&\sout{$78.61~\pm~nan$}&0&$\cellcolor{NiceOrange!25}\textbf{28.51}~\pm~nan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.014~\pm~0.028$&\scriptsize\sout{$1.090~\pm~nan$}&\scriptsize0&\scriptsize$0.983~\pm~nan$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{76.69}~\pm~9.27$&$\cellcolor{NiceBlue!25}\textbf{84.55}~\pm~\textbf{2.81}$&$\cellcolor{NiceBlue!25}\textbf{62.98}~\pm~\textbf{27.77}$&$27.90~\pm~\textbf{7.79}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.880~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$76.24~\pm~nan$&0&\sout{$\cellcolor{NiceOrange!25}\textbf{5.05}~\pm~nan$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.006~\pm~nan$&\scriptsize0&\scriptsize\sout{$1.024~\pm~nan$}&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{77.18}~\pm~\textbf{1.59}$&0&0&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize0&\scriptsize0&\scriptsize0\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$63.80~\pm~nan$&0&0&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.985~\pm~nan$&\scriptsize0&\scriptsize0&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{66.83}~\pm~\textbf{4.23}$&0&0&$\cellcolor{NiceBlue!25}\textbf{5.24}~\pm~nan$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize0&\scriptsize0&\scriptsize$0.932~\pm~nan$\\
\midrule\bottomrule
\end{tabular}

\caption{stack}
\end{table}





\newpage
\clearpage
\section{29 June 2023}


\begin{table}[h]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{36.73}~\pm~8.86$}&\sout{$37.39~\pm~\textbf{5.31}$}&\sout{$146.94~\pm~39.29$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.532~\pm~0.046$}&\scriptsize\sout{$1.321~\pm~0.584$}&\scriptsize\sout{$0.944~\pm~0.403$}\\
&$\rho_t=1$&metric&\sout{$22.26~\pm~7.12$}&\sout{$17.18~\pm~6.25$}&\sout{$\cellcolor{NiceOrange!25}\textbf{138.16}~\pm~3.68$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$2.203~\pm~1.072$}&\scriptsize\sout{$3.753~\pm~2.642$}&\scriptsize\sout{$1.635~\pm~0.588$}\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\cellcolor{NiceBlue!25}\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{34.16}~\pm~7.12$}&$33.80~\pm~5.96$&\sout{$\cellcolor{NiceGreen!25}\textbf{120.36}~\pm~nan$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.534~\pm~0.027$}&\scriptsize$0.500~\pm~0.004$&\scriptsize\sout{$0.473~\pm~nan$}\\
&$\rho_t=1$&metric&\sout{$32.18~\pm~\textbf{1.59}$}&$30.71~\pm~nan$&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.039~\pm~0.062$}&\scriptsize$0.999~\pm~nan$&\scriptsize0\\
&none&metric&$23.51~\pm~2.50$&$\cellcolor{NiceBlue!25}\textbf{39.84}~\pm~\textbf{5.91}$&$173.67~\pm~\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{95.35}~\pm~\textbf{0.23}$&$84.29~\pm~\textbf{1.28}$&$\cellcolor{NiceGreen!25}\textbf{101.99}~\pm~2.89$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.516~\pm~0.019$&\scriptsize$0.501~\pm~0.009$&\scriptsize$0.503~\pm~0.014$\\
&$\rho_t=1$&metric&\sout{$94.13~\pm~2.40$}&\sout{$74.15~\pm~nan$}&\sout{$104.24~\pm~4.92$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.621~\pm~0.957$}&\scriptsize\sout{$1.104~\pm~nan$}&\scriptsize\sout{$1.626~\pm~1.007$}\\
&none&metric&$94.85~\pm~0.40$&$\cellcolor{NiceBlue!25}\textbf{84.92}~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$67.24~\pm~48.71$}&$52.14~\pm~23.19$&\sout{$\cellcolor{NiceGreen!25}\textbf{107.80}~\pm~3.13$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.530~\pm~0.018$}&\scriptsize$0.499~\pm~0.001$&\scriptsize\sout{$0.612~\pm~0.168$}\\
&$\rho_t=1$&metric&\sout{$83.06~\pm~24.34$}&\sout{$45.67~\pm~26.11$}&\sout{$108.97~\pm~3.45$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.302~\pm~0.198$}&\scriptsize\sout{$1.071~\pm~0.041$}&\scriptsize\sout{$1.058~\pm~0.013$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{95.13}~\pm~\textbf{0.93}$&$\cellcolor{NiceBlue!25}\textbf{83.61}~\pm~\textbf{1.97}$&$108.80~\pm~\textbf{2.56}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$81.39~\pm~\textbf{11.64}$}&\sout{$62.60~\pm~18.23$}&\sout{$649.26~\pm~\textbf{0.32}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.294~\pm~0.044$}&\scriptsize\sout{$1.425~\pm~0.586$}&\scriptsize\sout{$2.921~\pm~0.336$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{92.88}~\pm~nan$&$\cellcolor{NiceBlue!25}\textbf{76.37}~\pm~\textbf{4.39}$&$\cellcolor{NiceBlue!25}\textbf{130.18}~\pm~1.06$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.225~\pm~nan$&\scriptsize$2.070~\pm~0.286$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{85.80}~\pm~4.78$}&\sout{$\cellcolor{NiceOrange!25}\textbf{74.94}~\pm~\textbf{0.32}$}&\sout{$518.65~\pm~254.39$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.103~\pm~0.132$}&\scriptsize\sout{$1.077~\pm~0.081$}&\scriptsize\sout{$2.017~\pm~0.500$}\\
&none&metric&$81.46~\pm~\textbf{1.41}$&$74.52~\pm~1.22$&$\cellcolor{NiceBlue!25}\textbf{130.88}~\pm~\textbf{4.40}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.217~\pm~0.008$&\scriptsize$1.211~\pm~0.004$&\scriptsize$1.168~\pm~0.065$\\
\midrule\bottomrule
\end{tabular}

\caption{task}
\end{table}



\begin{table}[h]
\centering
\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{40.49}~\pm~5.91$}&\sout{$\cellcolor{NiceGreen!25}\textbf{31.18}~\pm~\textbf{4.80}$}&\sout{$12.37~\pm~\textbf{1.60}$}&\sout{$4.76~\pm~0.20$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.716~\pm~0.193$}&\scriptsize\sout{$1.229~\pm~0.675$}&\scriptsize\sout{$0.651~\pm~0.032$}&\scriptsize\sout{$0.858~\pm~0.533$}\\
&$\rho_t=1$&metric&\sout{$36.92~\pm~\textbf{4.81}$}&\sout{$23.85~\pm~11.35$}&\sout{$8.09~\pm~5.90$}&\sout{$4.87~\pm~0.23$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$5.843~\pm~4.956$}&\scriptsize\sout{$1.612~\pm~0.339$}&\scriptsize\sout{$1.536~\pm~0.422$}&\scriptsize\sout{$1.467~\pm~0.056$}\\
&none&metric&$38.20~\pm~6.84$&$30.47~\pm~13.34$&$\cellcolor{NiceBlue!25}\textbf{12.90}~\pm~3.82$&$\cellcolor{NiceBlue!25}\textbf{5.06}~\pm~\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$35.00~\pm~\textbf{8.56}$&$31.71~\pm~6.72$&\sout{$\cellcolor{NiceGreen!25}\textbf{22.14}~\pm~12.37$}&\sout{$12.53~\pm~\textbf{2.23}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.511~\pm~0.028$&\scriptsize\sout{$0.547~\pm~0.040$}&\scriptsize\sout{$0.612~\pm~0.016$}\\
&$\rho_t=1$&metric&$34.83~\pm~11.24$&$\cellcolor{NiceOrange!25}\textbf{41.15}~\pm~\textbf{1.36}$&\sout{$17.69~\pm~\textbf{1.29}$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.011~\pm~0.040$&\scriptsize$0.999~\pm~0.002$&\scriptsize\sout{$1.041~\pm~0.014$}&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{39.06}~\pm~10.85$&$34.19~\pm~5.98$&$16.43~\pm~3.51$&$\cellcolor{NiceBlue!25}\textbf{15.59}~\pm~2.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&$75.10~\pm~10.53$&$85.76~\pm~\textbf{1.17}$&$86.43~\pm~\textbf{1.55}$&$\cellcolor{NiceGreen!25}\textbf{87.77}~\pm~\textbf{0.24}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.489~\pm~0.015$&\scriptsize$0.497~\pm~0.003$&\scriptsize$0.504~\pm~0.002$&\scriptsize$0.504~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$69.64~\pm~3.92$}&\sout{$80.28~\pm~4.78$}&\sout{$33.99~\pm~32.91$}&\sout{$37.85~\pm~36.66$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.043~\pm~0.077$}&\scriptsize\sout{$1.132~\pm~0.030$}&\scriptsize\sout{$1.182~\pm~0.050$}&\scriptsize\sout{$1.180~\pm~0.122$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{84.55}~\pm~\textbf{1.45}$&$\cellcolor{NiceBlue!25}\textbf{86.01}~\pm~2.48$&$\cellcolor{NiceBlue!25}\textbf{86.81}~\pm~3.05$&$85.96~\pm~0.61$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.701~\pm~0.003$&\scriptsize$0.700~\pm~0.001$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$68.37~\pm~15.23$}&$73.25~\pm~18.28$&\sout{$51.66~\pm~40.59$}&\sout{$5.08~\pm~\textbf{0.19}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.551~\pm~0.059$}&\scriptsize$0.518~\pm~0.029$&\scriptsize\sout{$0.543~\pm~0.018$}&\scriptsize\sout{$0.542~\pm~0.021$}\\
&$\rho_t=1$&metric&$41.98~\pm~\textbf{4.08}$&\sout{$83.61~\pm~4.09$}&\sout{$\cellcolor{NiceOrange!25}\textbf{71.89}~\pm~\textbf{22.71}$}&$\cellcolor{NiceOrange!25}\textbf{59.46}~\pm~28.38$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.014~\pm~0.028$&\scriptsize\sout{$1.117~\pm~0.117$}&\scriptsize\sout{$1.073~\pm~0.125$}&\scriptsize$0.982~\pm~0.017$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{76.69}~\pm~9.27$&$\cellcolor{NiceBlue!25}\textbf{84.82}~\pm~\textbf{2.35}$&$62.98~\pm~27.77$&$27.90~\pm~7.79$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.879~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$74.81~\pm~2.80$&\sout{$55.59~\pm~9.06$}&\sout{$5.06~\pm~\textbf{0.20}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{5.07}~\pm~\textbf{0.13}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.010~\pm~0.003$&\scriptsize\sout{$1.223~\pm~0.261$}&\scriptsize\sout{$1.056~\pm~0.054$}&\scriptsize\sout{$1.223~\pm~0.317$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{77.18}~\pm~\textbf{1.59}$&$\cellcolor{NiceBlue!25}\textbf{63.11}~\pm~\textbf{5.52}$&$\cellcolor{NiceBlue!25}\textbf{5.14}~\pm~0.29$&$4.98~\pm~0.17$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize$2.164~\pm~0.020$&\scriptsize$2.105~\pm~0.006$&\scriptsize$2.075~\pm~0.005$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{68.17}~\pm~\textbf{3.62}$&\sout{$55.65~\pm~24.91$}&\sout{$\cellcolor{NiceOrange!25}\textbf{29.64}~\pm~16.74$}&\sout{$5.08~\pm~\textbf{0.11}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.005~\pm~0.014$&\scriptsize\sout{$1.208~\pm~0.229$}&\scriptsize\sout{$1.085~\pm~0.040$}&\scriptsize\sout{$1.268~\pm~0.304$}\\
&none&metric&$66.83~\pm~4.23$&$\cellcolor{NiceBlue!25}\textbf{68.57}~\pm~\textbf{3.01}$&$18.86~\pm~\textbf{4.26}$&$\cellcolor{NiceBlue!25}\textbf{5.13}~\pm~0.19$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize$1.082~\pm~0.002$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.933~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{stack}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$11.32~\pm~\textbf{0.24}$&\sout{$12.37~\pm~\textbf{1.60}$}&\sout{$\cellcolor{NiceGreen!25}\textbf{486.38}~\pm~263.67$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.005$&\scriptsize\sout{$0.651~\pm~0.032$}&\scriptsize\sout{$0.897~\pm~0.478$}\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{11.50}~\pm~2.17$}&\sout{$8.09~\pm~5.90$}&\sout{$638.57~\pm~\textbf{0.51}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.529~\pm~0.218$}&\scriptsize\sout{$1.536~\pm~0.422$}&\scriptsize\sout{$1.291~\pm~0.260$}\\
&none&metric&$11.37~\pm~0.27$&$\cellcolor{NiceBlue!25}\textbf{12.90}~\pm~3.82$&$643.23~\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{31.84}~\pm~6.68$}&\sout{$\cellcolor{NiceGreen!25}\textbf{22.14}~\pm~12.37$}&\sout{$518.76~\pm~132.43$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.542~\pm~0.035$}&\scriptsize\sout{$0.547~\pm~0.040$}&\scriptsize\sout{$0.434~\pm~0.045$}\\
&$\rho_t=1$&metric&\sout{$25.12~\pm~nan$}&\sout{$17.69~\pm~\textbf{1.29}$}&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.975~\pm~nan$}&\scriptsize\sout{$1.041~\pm~0.014$}&\scriptsize0\\
&none&metric&$19.63~\pm~\textbf{6.60}$&$16.43~\pm~3.51$&$\cellcolor{NiceBlue!25}\textbf{500.04}~\pm~\textbf{94.49}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{96.45}~\pm~\textbf{0.24}$&$86.43~\pm~\textbf{1.55}$&$\cellcolor{NiceGreen!25}\textbf{122.36}~\pm~14.16$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.510~\pm~0.002$&\scriptsize$0.504~\pm~0.002$&\scriptsize$0.490~\pm~0.009$\\
&$\rho_t=1$&metric&\sout{$70.87~\pm~44.87$}&\sout{$33.99~\pm~32.91$}&\sout{$547.96~\pm~160.25$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.156~\pm~0.187$}&\scriptsize\sout{$1.182~\pm~0.050$}&\scriptsize\sout{$1.329~\pm~0.398$}\\
&none&metric&$95.61~\pm~0.38$&$\cellcolor{NiceBlue!25}\textbf{86.81}~\pm~3.05$&$648.25~\pm~\textbf{4.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.701~\pm~0.003$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$75.12~\pm~42.76$&\sout{$51.66~\pm~40.59$}&$640.17~\pm~\textbf{0.37}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.509~\pm~0.009$&\scriptsize\sout{$0.543~\pm~0.018$}&\scriptsize$0.517~\pm~0.017$\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{96.21}~\pm~0.48$}&\sout{$\cellcolor{NiceOrange!25}\textbf{71.89}~\pm~\textbf{22.71}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{473.95}~\pm~296.02$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.964~\pm~0.106$}&\scriptsize\sout{$1.073~\pm~0.125$}&\scriptsize\sout{$1.512~\pm~0.446$}\\
&none&metric&$96.19~\pm~\textbf{0.29}$&$62.98~\pm~27.77$&$644.18~\pm~0.59$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$10.99~\pm~0.84$}&\sout{$5.06~\pm~\textbf{0.20}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{650.22}~\pm~\textbf{1.85}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.769~\pm~0.840$}&\scriptsize\sout{$1.056~\pm~0.054$}&\scriptsize\sout{$1.405~\pm~0.192$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.20}~\pm~\textbf{0.08}$&$\cellcolor{NiceBlue!25}\textbf{5.14}~\pm~0.29$&$655.61~\pm~12.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.277~\pm~0.013$&\scriptsize$2.105~\pm~0.006$&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&\sout{$11.33~\pm~\textbf{0.25}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{29.64}~\pm~16.74$}&\sout{$\cellcolor{NiceOrange!25}\textbf{650.94}~\pm~1.37$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.619~\pm~0.780$}&\scriptsize\sout{$1.085~\pm~0.040$}&\scriptsize\sout{$1.248~\pm~0.010$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.73}~\pm~1.54$&$18.86~\pm~\textbf{4.26}$&$661.75~\pm~\textbf{0.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{task5}
\end{table}





\newpage
\clearpage
\section{3 July 2023}



\begin{table}[h]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{32.83}~\pm~2.69$&\sout{$39.62~\pm~7.89$}&$\cellcolor{NiceGreen!25}\textbf{116.96}~\pm~5.36$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.512~\pm~0.008$&\scriptsize\sout{$0.464~\pm~0.055$}&\scriptsize$0.481~\pm~0.015$\\
&$\rho_t=1$&metric&\sout{$26.27~\pm~2.85$}&\sout{$20.21~\pm~\textbf{6.92}$}&\sout{$171.15~\pm~15.82$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.109~\pm~0.057$}&\scriptsize\sout{$0.850~\pm~0.296$}&\scriptsize\sout{$1.052~\pm~0.019$}\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\cellcolor{NiceBlue!25}\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{32.39}~\pm~3.11$&$33.80~\pm~5.96$&$\cellcolor{NiceGreen!25}\textbf{120.78}~\pm~\textbf{0.49}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.518~\pm~0.030$&\scriptsize$0.500~\pm~0.004$&\scriptsize$0.498~\pm~0.001$\\
&$\rho_t=1$&metric&$30.82~\pm~\textbf{2.30}$&$30.71~\pm~nan$&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.011~\pm~0.017$&\scriptsize$0.999~\pm~nan$&\scriptsize0\\
&none&metric&$23.51~\pm~2.50$&$\cellcolor{NiceBlue!25}\textbf{39.84}~\pm~\textbf{5.91}$&$173.67~\pm~3.21$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{95.15}~\pm~\textbf{0.25}$&$84.29~\pm~\textbf{1.28}$&$\cellcolor{NiceGreen!25}\textbf{101.99}~\pm~2.89$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.502~\pm~0.010$&\scriptsize$0.501~\pm~0.009$&\scriptsize$0.503~\pm~0.014$\\
&$\rho_t=1$&metric&\sout{$93.48~\pm~3.15$}&\sout{$75.68~\pm~10.57$}&$102.42~\pm~2.15$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.040~\pm~0.040$}&\scriptsize\sout{$1.065~\pm~0.037$}&\scriptsize$1.000~\pm~0.034$\\
&none&metric&$94.85~\pm~0.40$&$\cellcolor{NiceBlue!25}\textbf{84.92}~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$74.26~\pm~42.18$&$52.03~\pm~18.94$&\sout{$108.18~\pm~\textbf{1.79}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.514~\pm~0.013$&\scriptsize$0.499~\pm~0.001$&\scriptsize\sout{$0.530~\pm~0.044$}\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{95.21}~\pm~\textbf{0.29}$}&\sout{$63.46~\pm~26.71$}&\sout{$\cellcolor{NiceOrange!25}\textbf{106.95}~\pm~2.41$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.073~\pm~0.080$}&\scriptsize\sout{$1.099~\pm~0.056$}&\scriptsize\sout{$1.032~\pm~0.023$}\\
&none&metric&$95.13~\pm~0.93$&$\cellcolor{NiceBlue!25}\textbf{83.61}~\pm~\textbf{1.97}$&$108.80~\pm~2.56$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$55.99~\pm~39.41$}&$61.87~\pm~11.08$&\sout{$649.13~\pm~1.74$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.973~\pm~0.048$}&\scriptsize$1.001~\pm~0.007$&\scriptsize\sout{$2.436~\pm~1.663$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{85.94}~\pm~\textbf{4.89}$&$\cellcolor{NiceBlue!25}\textbf{74.44}~\pm~\textbf{5.26}$&$\cellcolor{NiceBlue!25}\textbf{130.18}~\pm~\textbf{1.06}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.226~\pm~0.032$&\scriptsize$2.027~\pm~0.249$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$76.58~\pm~13.39$&$73.93~\pm~5.52$&\sout{$647.78~\pm~\textbf{1.70}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.005~\pm~0.033$&\scriptsize$1.019~\pm~0.026$&\scriptsize\sout{$1.761~\pm~1.288$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{80.12}~\pm~\textbf{1.80}$&$\cellcolor{NiceBlue!25}\textbf{74.77}~\pm~\textbf{1.12}$&$\cellcolor{NiceBlue!25}\textbf{130.88}~\pm~4.40$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.212~\pm~0.007$&\scriptsize$1.192~\pm~0.040$&\scriptsize$1.168~\pm~0.065$\\
\midrule\bottomrule
\end{tabular}

\caption{task}
\end{table}





\begin{table}[h]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$11.32~\pm~\textbf{0.24}$&\sout{$\cellcolor{NiceGreen!25}\textbf{21.74}~\pm~\textbf{2.81}$}&\sout{$639.84~\pm~2.46$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.005$&\scriptsize\sout{$0.524~\pm~0.013$}&\scriptsize\sout{$0.540~\pm~0.076$}\\
&$\rho_t=1$&metric&\sout{$10.92~\pm~0.61$}&$7.99~\pm~3.07$&$\cellcolor{NiceOrange!25}\textbf{638.51}~\pm~\textbf{0.59}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.049~\pm~0.075$}&\scriptsize$1.017~\pm~0.051$&\scriptsize$1.014~\pm~0.058$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.37}~\pm~0.27$&$12.90~\pm~3.82$&$643.23~\pm~0.94$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{29.89}~\pm~8.57$&$\cellcolor{NiceGreen!25}\textbf{27.00}~\pm~11.99$&$\cellcolor{NiceGreen!25}\textbf{255.62}~\pm~284.36$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.513~\pm~0.025$&\scriptsize$0.507~\pm~0.012$&\scriptsize$0.495~\pm~0.005$\\
&$\rho_t=1$&metric&0&$17.12~\pm~nan$&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize$1.016~\pm~nan$&\scriptsize0\\
&none&metric&$19.63~\pm~\textbf{6.60}$&$16.43~\pm~\textbf{3.51}$&$500.04~\pm~\textbf{94.49}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{96.45}~\pm~\textbf{0.24}$&$86.37~\pm~\textbf{1.27}$&$\cellcolor{NiceGreen!25}\textbf{117.37}~\pm~10.88$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.510~\pm~0.002$&\scriptsize$0.502~\pm~0.004$&\scriptsize$0.493~\pm~0.006$\\
&$\rho_t=1$&metric&\sout{$95.83~\pm~0.99$}&\sout{$64.15~\pm~28.64$}&$186.65~\pm~7.84$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.057~\pm~0.116$}&\scriptsize\sout{$1.025~\pm~0.039$}&\scriptsize$1.018~\pm~0.006$\\
&none&metric&$95.61~\pm~0.38$&$\cellcolor{NiceBlue!25}\textbf{86.81}~\pm~3.05$&$648.25~\pm~\textbf{4.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.701~\pm~0.003$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$75.12~\pm~42.76$&$66.67~\pm~\textbf{22.70}$&$640.15~\pm~\textbf{0.26}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.505~\pm~0.004$&\scriptsize$0.505~\pm~0.015$&\scriptsize$0.511~\pm~0.015$\\
&$\rho_t=1$&metric&\sout{$95.82~\pm~\textbf{0.06}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{68.80}~\pm~28.06$}&\sout{$\cellcolor{NiceOrange!25}\textbf{399.32}~\pm~278.22$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.158~\pm~0.085$}&\scriptsize\sout{$1.022~\pm~0.036$}&\scriptsize\sout{$1.180~\pm~0.120$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{96.19}~\pm~0.29$&$62.98~\pm~27.77$&$644.18~\pm~0.59$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{11.62}~\pm~0.27$}&\sout{$\cellcolor{NiceOrange!25}\textbf{5.14}~\pm~\textbf{0.13}$}&$\cellcolor{NiceOrange!25}\textbf{647.86}~\pm~13.26$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.679~\pm~1.270$}&\scriptsize\sout{$1.029~\pm~0.005$}&\scriptsize$0.994~\pm~0.049$\\
&none&metric&$11.08~\pm~\textbf{0.25}$&$5.14~\pm~0.29$&$655.61~\pm~\textbf{12.53}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.281~\pm~0.014$&\scriptsize$2.105~\pm~0.006$&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&\sout{$10.92~\pm~\textbf{0.51}$}&$\cellcolor{NiceOrange!25}\textbf{20.29}~\pm~17.66$&$\cellcolor{NiceOrange!25}\textbf{651.48}~\pm~1.90$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.663~\pm~1.332$}&\scriptsize$1.014~\pm~0.013$&\scriptsize$0.993~\pm~0.047$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.73}~\pm~1.54$&$17.68~\pm~\textbf{4.21}$&$661.75~\pm~\textbf{0.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{task5}
\end{table}




\begin{table}[h]
\centering
\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{42.42}~\pm~\textbf{4.46}$&$\cellcolor{NiceGreen!25}\textbf{39.15}~\pm~6.54$&\sout{$\cellcolor{NiceGreen!25}\textbf{21.74}~\pm~\textbf{2.81}$}&\sout{$4.79~\pm~\textbf{0.15}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.508~\pm~0.029$&\scriptsize$0.515~\pm~0.038$&\scriptsize\sout{$0.524~\pm~0.013$}&\scriptsize\sout{$0.473~\pm~0.017$}\\
&$\rho_t=1$&metric&\sout{$33.44~\pm~11.06$}&\sout{$8.15~\pm~\textbf{2.59}$}&$7.99~\pm~3.07$&\sout{$\cellcolor{NiceOrange!25}\textbf{5.43}~\pm~1.03$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.221~\pm~0.049$}&\scriptsize\sout{$1.088~\pm~0.035$}&\scriptsize$1.017~\pm~0.051$&\scriptsize\sout{$1.024~\pm~0.031$}\\
&none&metric&$38.20~\pm~6.84$&$30.47~\pm~13.34$&$12.90~\pm~3.82$&$5.06~\pm~0.16$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$35.00~\pm~\textbf{8.56}$&$31.67~\pm~6.73$&$\cellcolor{NiceGreen!25}\textbf{27.00}~\pm~11.99$&$\cellcolor{NiceGreen!25}\textbf{17.40}~\pm~6.75$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize$0.507~\pm~0.012$&\scriptsize$0.514~\pm~0.028$\\
&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{40.82}~\pm~8.56$&$\cellcolor{NiceOrange!25}\textbf{41.15}~\pm~\textbf{1.36}$&$17.12~\pm~nan$&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.008~\pm~0.006$&\scriptsize$0.999~\pm~0.002$&\scriptsize$1.016~\pm~nan$&\scriptsize0\\
&none&metric&$39.06~\pm~10.85$&$34.19~\pm~5.98$&$16.43~\pm~\textbf{3.51}$&$15.59~\pm~\textbf{2.31}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&\sout{$81.95~\pm~2.79$}&$85.76~\pm~\textbf{1.17}$&$86.37~\pm~\textbf{1.27}$&$\cellcolor{NiceGreen!25}\textbf{87.88}~\pm~\textbf{0.30}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.528~\pm~0.038$}&\scriptsize$0.497~\pm~0.003$&\scriptsize$0.502~\pm~0.004$&\scriptsize$0.503~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$73.24~\pm~4.54$}&$81.21~\pm~2.92$&\sout{$64.15~\pm~28.64$}&$75.87~\pm~4.04$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.038~\pm~0.066$}&\scriptsize$1.018~\pm~0.043$&\scriptsize\sout{$1.025~\pm~0.039$}&\scriptsize$0.991~\pm~0.006$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{84.55}~\pm~\textbf{1.45}$&$\cellcolor{NiceBlue!25}\textbf{86.01}~\pm~2.48$&$\cellcolor{NiceBlue!25}\textbf{86.81}~\pm~3.05$&$86.79~\pm~1.15$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.701~\pm~0.003$&\scriptsize$0.698~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$65.87~\pm~18.78$&$74.57~\pm~19.14$&$66.67~\pm~\textbf{22.70}$&\sout{$45.64~\pm~29.46$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.493~\pm~0.015$&\scriptsize$0.503~\pm~0.008$&\scriptsize$0.505~\pm~0.015$&\scriptsize\sout{$0.560~\pm~0.064$}\\
&$\rho_t=1$&metric&$48.37~\pm~\textbf{6.79}$&\sout{$\cellcolor{NiceOrange!25}\textbf{84.92}~\pm~\textbf{2.32}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{68.80}~\pm~28.06$}&\sout{$\cellcolor{NiceOrange!25}\textbf{53.95}~\pm~25.71$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.007~\pm~0.050$&\scriptsize\sout{$1.096~\pm~0.036$}&\scriptsize\sout{$1.022~\pm~0.036$}&\scriptsize\sout{$1.043~\pm~0.073$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{76.69}~\pm~9.27$&$84.82~\pm~2.35$&$62.98~\pm~27.77$&$27.90~\pm~\textbf{7.79}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.879~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$75.14~\pm~2.38$&$45.26~\pm~25.64$&\sout{$\cellcolor{NiceOrange!25}\textbf{5.14}~\pm~\textbf{0.13}$}&$4.87~\pm~\textbf{0.35}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.007~\pm~0.005$&\scriptsize$0.999~\pm~0.019$&\scriptsize\sout{$1.029~\pm~0.005$}&\scriptsize$0.989~\pm~0.005$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{77.18}~\pm~\textbf{1.59}$&$\cellcolor{NiceBlue!25}\textbf{61.42}~\pm~\textbf{5.64}$&$5.14~\pm~0.29$&$\cellcolor{NiceBlue!25}\textbf{5.24}~\pm~0.47$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize$2.074~\pm~0.181$&\scriptsize$2.105~\pm~0.006$&\scriptsize$1.956~\pm~0.206$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{68.17}~\pm~\textbf{3.62}$&$45.76~\pm~13.98$&$\cellcolor{NiceOrange!25}\textbf{20.29}~\pm~17.66$&$\cellcolor{NiceOrange!25}\textbf{5.38}~\pm~0.61$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.005~\pm~0.014$&\scriptsize$1.011~\pm~0.022$&\scriptsize$1.014~\pm~0.013$&\scriptsize$1.003~\pm~0.003$\\
&none&metric&$66.83~\pm~4.23$&$\cellcolor{NiceBlue!25}\textbf{68.57}~\pm~\textbf{3.01}$&$17.68~\pm~\textbf{4.21}$&$5.17~\pm~\textbf{0.18}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize$1.082~\pm~0.002$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.933~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{stack}
\end{table}





\newpage
\clearpage
\section{8 July 2023}




\begin{table}[h]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{31.96}~\pm~2.82$}&\sout{$39.59~\pm~5.54$}&\sout{$\cellcolor{NiceGreen!25}\textbf{116.32}~\pm~4.46$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.533~\pm~0.049$}&\scriptsize\sout{$0.539~\pm~0.064$}&\scriptsize\sout{$0.542~\pm~0.101$}\\
&$\rho_t=1$&metric&\sout{$29.87~\pm~3.72$}&\sout{$17.19~\pm~\textbf{4.46}$}&\sout{$166.02~\pm~8.47$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.949~\pm~0.108$}&\scriptsize\sout{$2.075~\pm~0.328$}&\scriptsize\sout{$1.782~\pm~0.084$}\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\cellcolor{NiceBlue!25}\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{33.20}~\pm~2.91$&$33.80~\pm~5.96$&$\cellcolor{NiceGreen!25}\textbf{120.78}~\pm~\textbf{0.49}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.007$&\scriptsize$0.500~\pm~0.004$&\scriptsize$0.498~\pm~0.001$\\
&$\rho_t=1$&metric&$30.39~\pm~nan$&$30.71~\pm~nan$&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.015~\pm~nan$&\scriptsize$0.999~\pm~nan$&\scriptsize0\\
&none&metric&$23.51~\pm~\textbf{2.50}$&$\cellcolor{NiceBlue!25}\textbf{39.84}~\pm~\textbf{5.91}$&$173.67~\pm~3.21$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&$95.15~\pm~0.25$&$84.29~\pm~\textbf{1.28}$&$\cellcolor{NiceGreen!25}\textbf{101.99}~\pm~2.89$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.502~\pm~0.010$&\scriptsize$0.501~\pm~0.009$&\scriptsize$0.503~\pm~0.014$\\
&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{95.32}~\pm~\textbf{0.17}$}&\sout{$79.83~\pm~3.39$}&$104.09~\pm~\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.076~\pm~0.120$}&\scriptsize\sout{$1.055~\pm~0.048$}&\scriptsize$1.001~\pm~0.007$\\
&none&metric&$94.85~\pm~0.40$&$\cellcolor{NiceBlue!25}\textbf{84.92}~\pm~2.05$&$103.78~\pm~0.21$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&\sout{$74.26~\pm~42.18$}&$52.03~\pm~18.94$&\sout{$\cellcolor{NiceGreen!25}\textbf{108.13}~\pm~1.83$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.521~\pm~0.023$}&\scriptsize$0.499~\pm~0.001$&\scriptsize\sout{$0.528~\pm~0.041$}\\
&$\rho_t=1$&metric&\sout{$95.07~\pm~\textbf{0.40}$}&\sout{$68.50~\pm~27.12$}&\sout{$110.32~\pm~\textbf{1.77}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.121~\pm~0.216$}&\scriptsize\sout{$1.090~\pm~0.076$}&\scriptsize\sout{$1.022~\pm~0.017$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{95.13}~\pm~0.93$&$\cellcolor{NiceBlue!25}\textbf{83.61}~\pm~\textbf{1.97}$&$108.80~\pm~2.56$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$47.72~\pm~35.20$}&\sout{$60.62~\pm~11.42$}&\sout{$649.12~\pm~1.48$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.900~\pm~0.885$}&\scriptsize\sout{$1.556~\pm~0.741$}&\scriptsize\sout{$3.318~\pm~0.579$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{85.94}~\pm~\textbf{4.89}$&$\cellcolor{NiceBlue!25}\textbf{74.44}~\pm~\textbf{5.26}$&$\cellcolor{NiceBlue!25}\textbf{130.18}~\pm~\textbf{1.06}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.226~\pm~0.032$&\scriptsize$2.027~\pm~0.249$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&\sout{$77.23~\pm~12.63$}&\sout{$72.89~\pm~6.44$}&\sout{$647.75~\pm~\textbf{0.47}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.064~\pm~0.137$}&\scriptsize\sout{$1.049~\pm~0.043$}&\scriptsize\sout{$3.444~\pm~0.157$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{80.12}~\pm~\textbf{1.80}$&$\cellcolor{NiceBlue!25}\textbf{74.77}~\pm~\textbf{1.12}$&$\cellcolor{NiceBlue!25}\textbf{133.78}~\pm~6.82$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.212~\pm~0.007$&\scriptsize$1.192~\pm~0.040$&\scriptsize$1.178~\pm~0.057$\\
\midrule\bottomrule
\end{tabular}

\caption{task}
\end{table}





\begin{table}[h]
\centering
\begin{tabular}{llrcccc}
\toprule
&&\textbf{depth}&1&3&5&7\\
\textbf{net}&\textbf{LSC}&&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&\sout{$\cellcolor{NiceGreen!25}\textbf{44.50}~\pm~\textbf{6.15}$}&\sout{$\cellcolor{NiceGreen!25}\textbf{37.20}~\pm~5.50$}&\sout{$\cellcolor{NiceGreen!25}\textbf{18.85}~\pm~\textbf{1.75}$}&\sout{$6.11~\pm~2.53$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$0.603~\pm~0.078$}&\scriptsize\sout{$0.559~\pm~0.068$}&\scriptsize\sout{$0.600~\pm~0.015$}&\scriptsize\sout{$0.705~\pm~0.196$}\\
&$\rho_t=1$&metric&\sout{$31.10~\pm~13.86$}&\sout{$9.28~\pm~\textbf{2.46}$}&\sout{$9.36~\pm~3.25$}&\sout{$\cellcolor{NiceOrange!25}\textbf{7.57}~\pm~1.83$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$2.630~\pm~0.500$}&\scriptsize\sout{$1.640~\pm~0.063$}&\scriptsize\sout{$1.406~\pm~0.052$}&\scriptsize\sout{$1.352~\pm~0.027$}\\
&none&metric&$38.20~\pm~6.84$&$30.47~\pm~13.34$&$12.90~\pm~3.82$&$5.06~\pm~\textbf{0.16}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.366~\pm~0.001$&\scriptsize$0.362~\pm~0.001$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.361~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$35.00~\pm~\textbf{8.56}$&$31.67~\pm~6.73$&$\cellcolor{NiceGreen!25}\textbf{27.00}~\pm~11.99$&$\cellcolor{NiceGreen!25}\textbf{20.01}~\pm~2.82$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.498~\pm~0.002$&\scriptsize$0.507~\pm~0.012$&\scriptsize$0.500~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$38.29~\pm~12.14$}&$\cellcolor{NiceOrange!25}\textbf{41.15}~\pm~\textbf{1.36}$&0&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.063~\pm~0.083$}&\scriptsize$0.999~\pm~0.002$&\scriptsize0&\scriptsize0\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{39.06}~\pm~10.85$&$34.19~\pm~5.98$&$16.43~\pm~\textbf{3.51}$&$15.59~\pm~\textbf{2.31}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.355~\pm~0.004$&\scriptsize$1.346~\pm~0.003$&\scriptsize$1.341~\pm~0.006$&\scriptsize$1.339~\pm~0.005$\\
\midrule
GRU&$\rho_t=0.5$&metric&$82.26~\pm~2.98$&$85.76~\pm~\textbf{1.17}$&$86.37~\pm~\textbf{1.27}$&$\cellcolor{NiceGreen!25}\textbf{87.88}~\pm~\textbf{0.30}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.506~\pm~0.015$&\scriptsize$0.497~\pm~0.003$&\scriptsize$0.502~\pm~0.004$&\scriptsize$0.503~\pm~0.003$\\
&$\rho_t=1$&metric&\sout{$71.84~\pm~2.51$}&$80.82~\pm~2.81$&$78.09~\pm~1.68$&$75.87~\pm~4.04$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.045~\pm~0.081$}&\scriptsize$1.014~\pm~0.042$&\scriptsize$1.019~\pm~0.028$&\scriptsize$0.991~\pm~0.006$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{84.55}~\pm~\textbf{1.45}$&$\cellcolor{NiceBlue!25}\textbf{86.01}~\pm~2.48$&$\cellcolor{NiceBlue!25}\textbf{86.81}~\pm~3.05$&$86.79~\pm~1.15$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.751~\pm~0.002$&\scriptsize$0.710~\pm~0.002$&\scriptsize$0.701~\pm~0.003$&\scriptsize$0.698~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$74.73~\pm~15.83$&$74.57~\pm~19.14$&$67.84~\pm~23.91$&\sout{$32.87~\pm~33.20$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.497~\pm~0.008$&\scriptsize$0.503~\pm~0.008$&\scriptsize$0.515~\pm~0.033$&\scriptsize\sout{$0.545~\pm~0.044$}\\
&$\rho_t=1$&metric&\sout{$44.83~\pm~\textbf{4.38}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{85.26}~\pm~\textbf{1.02}$}&$\cellcolor{NiceOrange!25}\textbf{70.59}~\pm~\textbf{22.26}$&\sout{$\cellcolor{NiceOrange!25}\textbf{56.51}~\pm~18.77$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.052~\pm~0.037$}&\scriptsize\sout{$1.159~\pm~0.049$}&\scriptsize$1.017~\pm~0.035$&\scriptsize\sout{$1.105~\pm~0.194$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{76.69}~\pm~9.27$&$84.82~\pm~2.35$&$62.98~\pm~27.77$&$27.90~\pm~\textbf{7.79}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.914~\pm~0.003$&\scriptsize$0.879~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.869~\pm~0.002$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&$75.14~\pm~2.38$&\sout{$56.79~\pm~20.71$}&\sout{$5.06~\pm~\textbf{0.20}$}&$4.82~\pm~\textbf{0.26}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.007~\pm~0.005$&\scriptsize\sout{$1.151~\pm~0.217$}&\scriptsize\sout{$1.026~\pm~0.006$}&\scriptsize$1.010~\pm~0.025$\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{77.18}~\pm~\textbf{1.59}$&$\cellcolor{NiceBlue!25}\textbf{61.42}~\pm~\textbf{5.64}$&$\cellcolor{NiceBlue!25}\textbf{5.13}~\pm~0.24$&$\cellcolor{NiceBlue!25}\textbf{5.22}~\pm~0.39$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.853~\pm~0.023$&\scriptsize$2.074~\pm~0.181$&\scriptsize$2.103~\pm~0.006$&\scriptsize$1.988~\pm~0.180$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{68.17}~\pm~\textbf{3.62}$&\sout{$42.39~\pm~20.98$}&$16.37~\pm~16.41$&$5.13~\pm~0.62$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.005~\pm~0.014$&\scriptsize\sout{$1.120~\pm~0.182$}&\scriptsize$1.018~\pm~0.014$&\scriptsize$1.014~\pm~0.020$\\
&none&metric&$66.83~\pm~4.23$&$\cellcolor{NiceBlue!25}\textbf{68.57}~\pm~\textbf{3.01}$&$\cellcolor{NiceBlue!25}\textbf{17.68}~\pm~\textbf{4.21}$&$\cellcolor{NiceBlue!25}\textbf{5.17}~\pm~\textbf{0.18}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.460~\pm~0.007$&\scriptsize$1.082~\pm~0.002$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.933~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{stack}
\end{table}






\begin{table}[h]
\centering
\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$11.32~\pm~\textbf{0.24}$&\sout{$\cellcolor{NiceGreen!25}\textbf{18.85}~\pm~\textbf{1.75}$}&\sout{$640.81~\pm~4.24$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.504~\pm~0.005$&\scriptsize\sout{$0.600~\pm~0.015$}&\scriptsize\sout{$0.624~\pm~0.167$}\\
&$\rho_t=1$&metric&\sout{$10.78~\pm~0.82$}&\sout{$9.36~\pm~3.25$}&\sout{$\cellcolor{NiceOrange!25}\textbf{638.84}~\pm~0.98$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.429~\pm~0.083$}&\scriptsize\sout{$1.406~\pm~0.052$}&\scriptsize\sout{$1.232~\pm~0.211$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.37}~\pm~0.27$&$12.90~\pm~3.82$&$643.23~\pm~\textbf{0.94}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.357~\pm~0.002$&\scriptsize$0.361~\pm~0.001$&\scriptsize$0.351~\pm~0.001$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{31.69}~\pm~9.48$&$\cellcolor{NiceGreen!25}\textbf{27.00}~\pm~11.99$&$\cellcolor{NiceGreen!25}\textbf{255.62}~\pm~284.36$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.505~\pm~0.009$&\scriptsize$0.507~\pm~0.012$&\scriptsize$0.495~\pm~0.005$\\
&$\rho_t=1$&metric&0&0&0\\
&\scriptsize&\scriptsize$\rho$&\scriptsize0&\scriptsize0&\scriptsize0\\
&none&metric&$19.63~\pm~\textbf{6.60}$&$16.43~\pm~\textbf{3.51}$&$500.04~\pm~\textbf{94.49}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.323~\pm~0.009$&\scriptsize$1.341~\pm~0.006$&\scriptsize$0.769~\pm~0.001$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{96.45}~\pm~\textbf{0.24}$&$86.37~\pm~\textbf{1.27}$&$\cellcolor{NiceGreen!25}\textbf{117.37}~\pm~10.88$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.510~\pm~0.002$&\scriptsize$0.502~\pm~0.004$&\scriptsize$0.493~\pm~0.006$\\
&$\rho_t=1$&metric&$96.11~\pm~0.68$&$78.09~\pm~1.68$&$186.65~\pm~7.84$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.996~\pm~0.064$&\scriptsize$1.019~\pm~0.028$&\scriptsize$1.018~\pm~0.006$\\
&none&metric&$95.61~\pm~0.38$&$\cellcolor{NiceBlue!25}\textbf{86.81}~\pm~3.05$&$648.25~\pm~\textbf{4.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.695~\pm~0.003$&\scriptsize$0.701~\pm~0.003$&\scriptsize$0.687~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$75.12~\pm~42.76$&$67.84~\pm~23.91$&$640.08~\pm~\textbf{0.26}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.507~\pm~0.006$&\scriptsize$0.515~\pm~0.033$&\scriptsize$0.511~\pm~0.012$\\
&$\rho_t=1$&metric&\sout{$96.06~\pm~\textbf{0.24}$}&$\cellcolor{NiceOrange!25}\textbf{70.59}~\pm~\textbf{22.26}$&\sout{$\cellcolor{NiceOrange!25}\textbf{389.06}~\pm~287.84$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.223~\pm~0.118$}&\scriptsize$1.017~\pm~0.035$&\scriptsize\sout{$1.215~\pm~0.211$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{96.19}~\pm~0.29$&$62.98~\pm~27.77$&$644.18~\pm~0.59$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.858~\pm~0.002$&\scriptsize$0.871~\pm~0.001$&\scriptsize$0.854~\pm~0.001$\\
\midrule\midrule
ALIF&$\rho_t=1$&metric&\sout{$\cellcolor{NiceOrange!25}\textbf{11.27}~\pm~0.27$}&\sout{$5.06~\pm~\textbf{0.20}$}&\sout{$\cellcolor{NiceOrange!25}\textbf{653.87}~\pm~\textbf{2.00}$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.938~\pm~0.910$}&\scriptsize\sout{$1.026~\pm~0.006$}&\scriptsize\sout{$1.169~\pm~0.177$}\\
&none&metric&$11.08~\pm~\textbf{0.25}$&$\cellcolor{NiceBlue!25}\textbf{5.13}~\pm~0.24$&$655.61~\pm~12.53$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.281~\pm~0.014$&\scriptsize$2.103~\pm~0.006$&\scriptsize$1.650~\pm~0.023$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&\sout{$11.05~\pm~\textbf{0.72}$}&$16.37~\pm~16.41$&\sout{$\cellcolor{NiceOrange!25}\textbf{652.52}~\pm~1.29$}\\
&\scriptsize&\scriptsize$\rho$&\scriptsize\sout{$1.916~\pm~1.101$}&\scriptsize$1.018~\pm~0.014$&\scriptsize\sout{$1.395~\pm~0.610$}\\
&none&metric&$\cellcolor{NiceBlue!25}\textbf{11.73}~\pm~1.54$&$\cellcolor{NiceBlue!25}\textbf{17.68}~\pm~\textbf{4.21}$&$661.75~\pm~\textbf{0.75}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.090~\pm~0.005$&\scriptsize$0.979~\pm~0.002$&\scriptsize$0.973~\pm~0.001$\\
\midrule\bottomrule
\end{tabular}

\caption{task5}
\end{table}

% 11 -> 8
\begin{table*}[h]
\centering

\begin{tabular}{llrccc}
\toprule
&&\textbf{task}&\textbf{sl-MNIST}$\uparrow$&\textbf{SHD}$\uparrow$&\textbf{PTB}$\downarrow$\\
\textbf{net}&\textbf{LSC}&&&&\\
\\\toprule\midrule
RNN\,$\sigma$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{29.38}~\pm~6.65$&$34.66~\pm~8.30$&$\cellcolor{NiceGreen!25}\textbf{116.81}~\pm~7.31$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.492~\pm~0.008$&\scriptsize$0.496~\pm~0.007$&\scriptsize$0.497~\pm~0.003$\\
&$\rho_t=1$&metric&$26.98~\pm~3.29$&$36.37~\pm~\textbf{5.23}$&$276.09~\pm~244.64$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.992~\pm~0.142$&\scriptsize$1.019~\pm~0.019$&\scriptsize$0.981~\pm~0.335$\\
&none&metric&$29.02~\pm~\textbf{2.00}$&$\textbf{46.40}~\pm~12.12$&$641.65~\pm~\textbf{1.76}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.354~\pm~0.002$&\scriptsize$0.363~\pm~0.001$&\scriptsize$0.353~\pm~0.000$\\
\midrule
RNN\,$ReLU$&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{28.12}~\pm~3.41$&$35.46~\pm~10.64$&$\cellcolor{NiceGreen!25}\textbf{158.79}~\pm~10.43$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.500~\pm~0.003$&\scriptsize$0.508~\pm~0.003$&\scriptsize$0.516~\pm~0.002$\\
&$\rho_t=1$&metric&$24.80~\pm~5.44$&$33.34~\pm~\textbf{4.90}$&$167.83~\pm~13.57$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.997~\pm~0.009$&\scriptsize$0.945~\pm~0.177$&\scriptsize $1.019~\pm~0.004$\\
&none&metric&$23.51~\pm~\textbf{2.50}$&$\textbf{39.84}~\pm~5.91$&$173.67~\pm~\textbf{3.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.317~\pm~0.011$&\scriptsize$1.349~\pm~0.007$&\scriptsize$0.760~\pm~0.004$\\
\midrule
GRU&$\rho_t=0.5$&metric&$\cellcolor{NiceGreen!25}\textbf{95.28}~\pm~\textbf{0.17}$&$\cellcolor{NiceGreen!25}\textbf{85.58}~\pm~\textbf{1.35}$&$\cellcolor{NiceGreen!25}\textbf{103.12}~\pm~0.25$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.482~\pm~0.020$&\scriptsize$0.491~\pm~0.006$&\scriptsize$0.499~\pm~0.001$\\
&$\rho_t=1$&metric&$95.04~\pm~0.75$&$84.40~\pm~2.21$&$103.41~\pm~0.78$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.004$&\scriptsize$1.003~\pm~0.005$&\scriptsize$1.002~\pm~0.004$\\
&none&metric&$94.85~\pm~0.40$&$84.92~\pm~2.05$&$103.78~\pm~\textbf{0.21}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.710~\pm~0.004$&\scriptsize$0.719~\pm~0.002$&\scriptsize$0.694~\pm~0.002$\\
\midrule
LSTM&$\rho_t=0.5$&metric&$95.21~\pm~\textbf{0.24}$&\cellcolor{NiceGreen!25}$\textbf{84.48}\pm \textbf{0.97}$&$\cellcolor{NiceGreen!25}\textbf{108.83}\pm \textbf{1.65}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.503~\pm~0.006$&\scriptsize$0.516~\pm~0.026$&\scriptsize$0.511~\pm~0.016$\\
&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{95.60}~\pm~0.40$&$82.87~\pm~2.75$&$109.93~\pm~1.90$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.985~\pm~0.038$&\scriptsize$0.997~\pm~0.014$&\scriptsize$1.000~\pm~0.018$\\
&none&metric&$95.21~\pm~0.95$&$83.61~\pm~1.97$&$108.93~\pm~2.83$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.876~\pm~0.005$&\scriptsize$0.887~\pm~0.002$&\scriptsize$0.847~\pm~0.003$\\
\midrule\midrule
ALIF$_+$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{86.45}~\pm~\textbf{3.30}$&$\cellcolor{NiceOrange!25}\textbf{83.18}~\pm~\textbf{0.95}$&$\cellcolor{NiceOrange!25}\textbf{129.82}\pm\textbf{0.96}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.988~\pm~0.003$&\scriptsize$1.001~\pm~0.001$&\scriptsize$0.978\pm0.208$\\
&none&metric&$86.38~\pm~5.16$&$70.26~\pm~7.12$&$130.18~\pm~1.06$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$2.225~\pm~0.033$&\scriptsize$1.748~\pm~0.016$&\scriptsize$1.690~\pm~0.022$\\
\midrule
ALIF$_{\pm}$&$\rho_t=1$&metric&$\cellcolor{NiceOrange!25}\textbf{82.05}~\pm~6.26$&$\cellcolor{NiceOrange!25}\textbf{73.98}~\pm~\textbf{3.75}$&\cellcolor{NiceOrange!25}$\textbf{125.80}\pm\textbf{0.59}$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$0.999~\pm~0.001$&\scriptsize$1.000~\pm~0.000$&\scriptsize$0.981~\pm~0.002$\\
&none&metric&$81.42~\pm~\textbf{1.17}$&$68.20~\pm~6.85$&$130.54~\pm~5.09$\\
&\scriptsize&\scriptsize$\rho$&\scriptsize$1.212~\pm~0.007$&\scriptsize$1.130~\pm~0.003$&\scriptsize$1.094~\pm~0.002$\\
\midrule\bottomrule
\end{tabular}

\caption{\textbf{Pre-training $d$-RNN to stability improves training across tasks and neuron models.} The network preparation by pre-training to stability, generally helps performance, with $\rho_t=0.5$ (green) generally being preferable over $\rho_t=1$ (orange) across tasks and networks, with networks of depth $d=2$. Here we report the test set results across three different tasks. Metrics are accuracy for sl-MNIST and SHD, the higher the better ($\uparrow$), and perplexity for PTB, the lower the better ($\downarrow$). The non-differentiable networks, were often unable to reach a target norm of $\rho_t=0.5$, but the preparation to $\rho_t=1$ was still always beneficial.}
\label{tab:truelsctask}
\end{table*}



% This might become useful when I have good results on JAX


\begin{table*}
\centering
\begin{tabular}{lcccccc>{\columncolor[gray]{0.95}}c}
% \toprule
\textbf{Method} & \textbf{sCIFAR} & \textbf{ListOps} & \textbf{Text} & \textbf{Retrieval} & \textbf{Pathfinder} & \textbf{PathX} & \textbf{Average} \\
\hline
S4D \cite{orvieto2023resurrecting} & \textbf{91.5} (0.2) & 60.2 (0.3) & 86.4 (0.0) & 89.5 (0.0) & 94.2 (0.3) & 97.5 (0.0) & 86.6\\
S5 \cite{orvieto2023resurrecting} & 88.8 (0.1) & 58.5 (0.3) & 86.2 (0.1) & 88.9 (0.0) & \textbf{95.7} (0.1) & 96.0 (0.1) & 85.7 \\
S4 \cite{gu2022efficiently} & 91.1 & 59.6 & 86.8 & 90.9 & 94.2 & 96.4 & 86.5 \\
S4D-LegS \cite{gu2022parameterization} & 89.9 & \textbf{60.5} & 86.2 & 89.5 & 93.1 & 91.9 & 85.2 \\
S5 \cite{smith2023simplified} & 88.0 & 62.2 & 89.3 & \textbf{91.4} & 95.3 & \textbf{98.6} & \textbf{87.8}\\
\hline
LRU \cite{orvieto2023resurrecting} & 89.0 (0.1) & 60.2 (0.8) & \textbf{89.4} (0.1) & 89.9 (0.1) & 95.1 (0.1) & 94.2 (0.4) & 86.2\\
\hline
\hspace{3cm}(ours) &  &  &  &  &  &  &  \\
S5 & - & - & - & - & - & - & - \\
LRU & - & - & - & - & - & - & - \\
LRU + LSC $\rho_t=1$ & - & - & - & - & - & - & - \\
LRU + LSC $\rho_t=0.5$  & - & - & - & - & - & - & - \\
\st{LRU + LSC $\overline{\rho}_t=0.5$}  & - & - & - & - & - & - & - \\
LRU  + clip& - & - & - & - & - & - & - \\
\st{LRU + LSC $\rho_t=1$  + clip} & - & - & - & - & - & - & - \\
\st{LRU + LSC $\rho_t=0.5$  + clip} & - & - & - & - & - & - & - \\
\st{LRU + LSC $\overline{\rho}_t=0.5$  + clip} & - & - & - & - & - & - & - \\
% \midrule
% \bottomrule \\
\end{tabular}
\end{table*}


==> sections/related_work.tex <==
\section{Related Work}


